The clustering of galaxies in the SDSS-III Baryon Oscillation Spectroscopic Survey: Effect of smoothing of density field on reconstruction and anisotropic BAO analysis

The reconstruction algorithm introduced by \cite{Eis07}, which is widely used in clustering analysis, is based on the inference of the first order Lagrangian displacement field from the Gaussian smoothed galaxy density field in redshift space. The \modif2{smoothing scale} applied to the density field affects the inferred displacement field that is used to move {the galaxies}, and partially \modif2{erases} the nonlinear evolution {of the density field}. In this article, we explore this crucial step \modif2{in} the reconstruction algorithm. We study the performance of the reconstruction technique using two metrics: first, we study the performance using the anisotropic clustering, extending previous studies focused on isotropic clustering; second, we study its effect on the displacement field. We find that smoothing has a strong effect in the quadrupole of the correlation function and affects the accuracy and precision \modif2{with} which we can measure $D_A (z)$ and $H(z)$. We find that the optimal smoothing scale to use in the reconstruction algorithm applied to BOSS-CMASS is between 5-10 $h^{-1}$Mpc. Varying from the "usual" 15$h^{-1}$Mpc to $5 h^{-1}$Mpc \modif2{shows} $\sim$ 0.3\% variations in $D_A(z)$ and $\sim$ 0.4\% $H(z)$ and uncertainties are also reduced by 40\% and 30\% respectively. We also find that the accuracy of velocity field reconstruction depends strongly on the smoothing scale used for the density field. We measure the bias and uncertainties associated with different choices of smoothing length.

==> smoothtest_July_seb_ant_v3_seb_antonio.tex <==
\section{Introduction}
% \rr{REFEREE COMMENT: The first sentence is not introductory enough. Which density field?}\\
%\bb{Added an introductory paragraph here about BAO}\\
{\bf The Baryon Acoustic Oscillations (BAO) is without any doubt a robust and promising probe for decrypting dark energy (DE). Furthermore, BAO plays a central role in current and future DE experiments devoted to understand cosmic expansion \citep{DESI,Euclid,WFIRST}. The BAO signature corresponds to the imprint left by sound waves generated during the early Universe in the baryon-photon fluid and propagated until the time of decoupling, when the photon decouples from baryons and the sound waves get frozen. While the linear physics of these baryon acoustic oscillations is well understood, 
the nonlinear evolution of the matter density field leads to a coupling of the Fourier-modes, which generates a damping of the Baryonic Acoustic Oscillations (BAO) in the power spectrum of galaxies as well as a shift in the BAO peak position.}
The damping in the power spectrum translates to a blurring of the baryonic acoustic peak in the correlation function of galaxies in configuration space. 
%This reduction of the contrast in the baryonic acoustic feature generates an increase in the uncertainty in the derived BAO distance measurements.
{\bf This reduction of the contrast in the baryonic acoustic feature increases the uncertainty in the BAO distance derived from measurements.}

The major contribution to this damping comes from the bulk flows that shift the positions of the galaxies from the linear theory prediction \citep{Eis07}. 
Early work on reconstruction \citep{Eis06,PadWhiCoh} suggested that this effect could be partially reversed using the density field to infer the gravitational potential that sources the movement of the galaxies. 
%\sout{Undoing these bulk flows allows one to increase the signal-to-noise in the BAO feature and reduces the errors in the distance measurements.} \rr{REFEREE COMMENT: Undoing these bulk flows"-> doesn't really make sense}
%The damping of the BAO feature is mostly driven by the %large scale modes and bulk flows and cluster formation \citep{Eis06,Eis07} that moves the original position of the matter by around ~10 Mpc/h because of non linear colapse. Undoing these bulk flows
{\bf Running backwards the gravitational flow restores the BAO feature and reduce the errors in the distance measurements.}
%\rr{REFEREE COMMENT: Also isnÕt reconstruction about moving the randoms too, so this bulk flow reversal is not the entire picture}.% \bb{We explained the reconstruction algorithm in the section \label{sec:rec}, Write HERE a convincing phrase to state here is not the right place for this explanation} %NEEDS TO BE COMPLETED BUT HERE? OR LATER}

 \cite{Pad12} extended the methodology  from \cite{Eis07} by applying reconstruction to galaxy {\bf catalogues}. Since then, reconstruction has been successfully applied to galaxy clustering analysis in different galaxy {\bf catalogues} and surveys. In most of the cases\footnote{{\bf Few samples  in SDSS galaxy {\bf catalogues}, such as DR9 CMASS sample \citep{And12} and the DR10 LOWZ sample \citep{Toj14}, reported  almost no improvement, but such results are consistent with the expected results using mock galaxy {\bf catalogues} given the already small initial error compared to the average of the pre-reconstruction {\bf catalogues}.}}, reconstruction is shown to increase the precision of the measurements in the samples analysed \citep{Pad12,And12,And13, And14,Toj14,Kaz14, Ross14} with up to $\sim$ 45-percent improvement in the error bars in certain samples. These results are responsible for reconstruction becoming an essential part of the clustering analysis.

 {\bf While reconstruction has shown to be a successful mechanism to obtain more precise BAO measurements, the performance of reconstruction algorithm is still under intense investigation. }
{\bf Given the current precision in BAO distance measurements, the study of the associated uncertainties becomes essential for current and future surveys.} Some efforts to understand reconstruction analytically have appeared in the literature: \cite{PadWhiCoh} provided an analytic formalism within the context of Lagrangian perturbation theory; \cite{Noh09} extended this formalism for biased tracers. \cite{white15} developed the formalism to describe post-reconstruction correlation functions within the Zeldovich Approximation. \cite{xu12} studied the isotropic effects of reconstruction while \cite{And12} studied the anisotropic  effects. 
Reconstruction performance also has been studied using N-body simulations \citep{Seo06,Seo10}. \cite{Pad12} provides a first exploration of the robustness of reconstruction methodology against different implementation choices in the isotropic BAO analysis.  \cite{bur14} and, \cite{bur15} {\bf provided} a more detailed empirical study of the systematics (density dependence, geometry effects, RSD corrections) {\bf in the} reconstruction algorithm. Both of these studies concentrated on the reconstruction effects on isotropic clustering. \cite{Var14} also studied the results post-reconstruction but focused on anisotropic fitting systematics. 

The reconstruction algorithm requires an estimate of the density field, {\bf in order to} estimate the displacement field using the Zel'dovich approximation \citep{Zel}. The density field is usually smoothed with a Gaussian kernel \citep{Pad12,And12,And13,And14},
whose width sets the scale that will source the displacement field.  
 A large smoothing scale could erase cosmological information, reducing the effect of reconstruction. Furthermore, information in the regions sourcing the nonlinear growth will be suppressed. On the other hand, a too small smoothing scale increases the noise in the linear density field. 
 As it is implemented now, the smoothing scale is a free parameter. In Table \ref{tab:smoothingPast} we summarise different studies related to the smoothing scale; we show the references, scales explored, the method of analysis (i.e configuration of Fourier space) and the \sout{kind of} mocks used for the study. \cite{whi10} studied the shot noise effect on reconstruction and found that for low density tracers, 
% a large smoothing scale performs better to define the shifts in the BAO position.
% \rr{REFEREE COMMENT: large smoothing performs better to define the shifts" this doesn't really make sense.}
 {\bf a large smoothing scale performs better in terms of isotropic clustering as it generates a smaller shift in the  BAO measurement.}
 Most BAO clustering analyses \citep{Eis07,Pad12,And12,And13,And14} use a Gaussian smoothing kernel of $R$ = 10-20 $h^{-1}$ Mpc. Some small deviations from this smoothing length have been shown not to alter the results (see Appendix B of Anderson et al. 2012 and Padmanabhan et al. 2012a). \cite{bur14} studied the impact of the smoothing length on the isotropic BAO analysis. They found that the bias in the measurement of the isotropic dilation parameter $\alpha$ is reduced using a smoothing scale of $15 h^{-1}$ Mpc  for CMASS and a smoothing scale of $10h^{-1}$ Mpc for LOWZ. 
 In this paper we extend those analyses to present a study of the effect of smoothing scale on reconstruction performance in the anisotropic BAO analysis.  
\begin{table*}
\begin{center}
\caption{Smoothing scales tested with simulations } 
\label{tab:smoothingPast}
\begin{tabular}{@{}lcccccccccc}
\hline
Reference &$R$'s ($h^{-1}$ Mpc)& Best $R$&observable&Mock {\bf catalogues}\\
\hline
\cite{Pad12}&10,15, 20, 25 & 15 &$\xi_0(r)$& N-body \\
\cite{bur14,bur15} &5,8 10 ,15 20 ,40 & 15&$P(k)$& 2LPT Mocks \\
\cite{bur15} &5 10 ,15 & -&$\Psi(r)$& 2LPT Mocks \\
\cite{Noh09}&5,10, 15, 20, 25, 30&-&$\Psi(r)$&N-body\\
 \hline
\\[-1.5ex]
\end{tabular}
\end{center}
\end{table*}

The motivation for this study is illustrated in Figure \ref{fig:MeanDiffSimsImp}. We show the mean and root mean square (RMS) of the correlation function from 100 mock {\bf catalogues} before and after reconstruction (hereafter, pre- and post- reconstruction). The different colours are different kinds of mock {\bf catalogues}.
Darker shades are pre-reconstruction, and lighter shades are post-reconstruction {\bf catalogues}. In blue are the PTHALOS mock {\bf catalogues} used for the analysis of the Baryonic Oscillations Spectroscopic Survey (BOSS) \citep{Daw13} of Sloan Digital Sky Survey III (SDSS-III) \citep{Eis11} galaxy samples Data Releases 9, 10 and 11 (DR9, DR10, DR11). PTHALOS mocks are based on second order Lagrangian Perturbation Theory \citep{man13}. In green are the Quick Particle Mesh mock {\bf catalogues} used to analyse BOSS DR12 based on low resolution N-body simulations combined with HOD models for populating halos with galaxies. Finally in red are the MD-PATCHY (Kitaura et al, 2015; %\citep[{{Kitaura et al }(2015)}][
companion paper) %]{Kit15} 
mocks based on Augmented Lagrangian Perturbation Theory and stochastic bias prescriptions generated for BOSS DR12 analysis.
In all types of simulations, reconstruction succeeded to 1) sharpen the BAO feature in the monopole, and 2) reduce the quadrupole to be consistent with zero at large scales when we remove the redshift space distortions.  
 However, different trends {\bf are} observed in the post-reconstruction mean correlation function, {\bf depending} on the details of the reconstruction implementation and/or the simulations.   
The PTHALOS mocks show a slightly positive quadrupole post-reconstruction compared with QPM and PATCHY, which show a slightly negative quadrupole. 
We note that the implementation used in PTHALOS is from \cite{Pad12}, while the one used in the QPM and PATCHY mocks is ours; the cosmology of the three different simulations is also different. 
 A perfect reconstruction would remove large-scale anisotropy from the correlation function when we remove the redshift space distortions from the {\bf catalogues}. However, in the case plotted, there is a residual anisotropy in the quadrupole at large scales (negative or positive) showing that the reconstruction is not perfect.  The aim of this article is to disentangle the relation of this residual with the smoothing length and check the effect of the smoothing length in the BAO anisotropic post-reconstruction results. 
 
In this work the main metric we use to evaluate the performance of reconstruction is the anisotropic BAO fits. Additionally we explore the smoothing effects on the correlation functions and on the displacement field %\gr{\sout{; however, the last two will only serve to understand}}
 {\bf as a way  of understanding} the anisotropic fit results. We find that the smoothing length affects the quadrupole amplitude. Furthermore, we find that the differences in the amplitude also depend on the implementation. However, we show that the differences in the amplitude of the quadrupole do not determine the anisotropic results. We also explore if the origin of the improvement in anisotropic fits was related to a better estimate of the displacement field.

This study addresses a crucial point in current BAO analysis, especially in the context of final data release of BOSS galaxy data. The results we found are BOSS specific; however, we include a section with some additional tests to explore how these conclusions scale with the bias and the number density so that the results could be generalised to other surveys.
 
The layout of this paper is as follows. We introduce the reconstruction implementation in Section \ref{sec:rec}. We present the simulations used in our study in Section \ref{sec:sim} and the analysis methods for anisotropic BAO measurements in Section \ref{sec:method}. We then present the results in Sections \ref{sec:fits} and \ref{sec:disp}. Section \ref{sec:fits} presents the effect of the smoothing in anisotropic BAO fitting results and Section \ref{sec:disp} presents the effect of smoothing on the displacement estimation accuracy. We conclude in Section \ref{sec:con}.


\begin{figure}
   \centering    
   \includegraphics[width=3.6in]{Meanx0x2_ALL_final.pdf}%{Meanx0_ALL_final_PTHALOS.pdf}%
  \caption{Performance of reconstruction tested in different kinds of sky-type mock {\bf catalogues}. We show the mean of monopole [top panel], quadrupole [bottom panel] from 100 mocks pre-reconstruction and post-reconstruction. The different colours are different kinds of mock {\bf catalogues}: darker shades are pre-reconstruction and lighter shades are post-reconstruction {\bf catalogues}. In blue are the PTHALOS  \citep{man13}. In green are the Quick Particle Mesh \citep{QPM} . In red are the PATCHY (Kitaura et al 2015; companion paper). For the monopole we get pretty similar results in the BAO fitting range. However, in all cases the post-reconstruction quadrupole  is not exactly zero; there is an extra correlation (negative or positive).  
     The purpose of this work is to disentangle the relation of this residual with the smoothing length and check the effect of the smoothing length on the BAO anisotropic post-reconstruction results.}
   \label{fig:MeanDiffSimsImp}
\end{figure}

\section{Reconstruction Basic Algorithm}\label{sec:rec}

The algorithm of density field reconstruction has been described in  \cite{Eis07,Pad12, bur14}. %, Seo10}. \sout{many references}
{\bf We describe the most general algorithm applied to biased tracers considering redshift space distortions, the angular and radial mask of the data.} We focus on the part where the smoothing scale enters the reconstruction algorithm.
The algorithm proposed by \cite{Eis07} can be directly summarised as follows: 
\begin{itemize}
\item Estimate the over-density field from the galaxy positions using an interpolation method. We are using Nearest Grid Point (NGP) interpolation method. 
\item Smooth the over-density field using a Gaussian filter with smoothing scale R in order to eliminate high $k$ non-linearities (small scales).
\begin{equation}
W_G(k)=\exp(-R^2 k^2/2)
\end{equation}
\item Solve the Eq.(\ref{Ap:ZAg}) using the Zeldovich approximation. 
\begin{equation}\label{Ap:ZAg}
\nabla \cdot \vec{\Psi}+f \nabla \cdot (\vec{\Psi} \cdot \vec{r}) \hat{r}=-\frac{\delta_g}{b}.
%\nabla \cdot \vec{\Psi}(r)+f \nabla \cdot (\vec{\Psi}(r) \cdot \vec{r}) \hat{r}=-\frac{\delta(r)}{b}.
\end{equation}
where $\vec{\Psi}$ is the displacement field, $\vec{r}$ the galaxy position, $\delta_g$ the galaxy contrast of density and $b$ the bias.

{\bf We can solve Eq.(\ref{Ap:ZAg}) in configuration space following a finite differences approach \citep{Pad12} or in Fourier space \citep{bur14}.}
{\bf In order to solve it in Fourier space,  it is assumed that $(\vec{\Psi} \cdot \hat{r})\hat{r}$
%the divergence of the displacement field 
is irrotational, which enables us to approximate it as the gradient of a potential field, i.e  solve Eq.(\ref{Ap:ZAg}).}
%to solve Eq.(\ref{Ap:ZAg}) 
%A similar approach is used in \cite{bur14} where it is assumed that the divergence of the displacement field is irrotational, which enables us to solve Eq.(\ref{Ap:ZAg}) in Fourier space. 
{\bf The implications of this approximation were explored in \cite{bur15}  showing that the displacement field is underestimated when the irrotational component is neglected, suggesting an empirical formula to correct this effect.} %\sout{in terms of the displacement field}

{\bf In our implementation we also use the Fourier transform method  to solve for the displacements. However, we follow a simpler approach by neglecting the effect of the RSD when measuring the density field, leading to this equation :}\begin{equation} \nabla \cdot \vec{\Psi}=-\frac{\delta_g}{b}.\end{equation} {\bf instead of solving equation \ref{Ap:ZAg}. }, and we estimate the displacement field by:
\begin{equation}
%\vec{\Psi}(k)=\text{IFFT} \left [ \frac{-i\vec{k}\delta_g(k)}{k^2b}\right ].
\vec{\Psi}=\text{IFFT} \left [ \frac{-i\vec{k}\delta_g(\vec{k})}{k^2b}\right ].
\end{equation}

We verify that this choice does not affect the conclusions of the tests performed (see Appendix \ref{ap:imp}). 
The effect of applying different RSD corrections on the  displacement field %for accounting for the fact that we measure the density in redshift space 
is performed in \cite{bur15}. 
A study of the effects of applying different RSD corrections  in terms of anisotropic fits is performed in Vargas-Maga\~na (in preparation).  
\item {\bf Once the displacement is computed, we move the particles positions by the corresponding displacement, $-\vec{\Psi}$, to approximate their initial Lagrangian positions.} This step provides the short-scale modes of the reconstructed density \citep{PadWhiCoh, Noh09}. 
\item Move an additional $\vec{\Psi}_{RSD}$ if we want to eliminate the redshift space distortions at large scales in the catalogue: 
\begin{equation}
%\vec{\Psi}_{RSD}(r)=-f (\vec{\Psi}(r) \cdot  \hat{r}) \; \hat{r}. 
\vec{\Psi}_{RSD}=-f (\vec{\Psi} \cdot  \hat{r}) \; \hat{r}. 
\end{equation}
\item Generate a uniform random sample and move the particles using the displacement field previously estimated from data. This step provides us the large-scale modes of the reconstructed density.
%\sout{The reconstructed density field is the sum of the two contributions of the large- and small-scale modes. The small-scale motions stay in the galaxy field, while the large-scale clustering signal moves into the random catalogue.}
\end{itemize}
The  2-point correlation post-reconstruction is then  defined as:
%\sout{ The two components of the reconstructed density will be taken into account in the 2-point correlation estimator}:
\begin{equation}
\xi_{LS}(r,\mu)=\frac{DD(r,\mu)-2DS(r, \mu)+SS(r, \mu)}{RR(r, \mu)},
\end{equation}
where $D$ accounts for the data, $S$ for the ``shifted'' random sample and $R$ for the ``non-shifted" random sample.  The $DD$ describes the pair counts per r-$\mu$ bin with data-data, $SS$ the same for the shifted random pair-counts and $RR$ for the non-shifted randoms. $DS$ will be the pair-counts per r-$\mu$ bin taking  one point from data and one from the shifted random set.

{\bf The current reconstruction algorithm treats separately the small and large scale modes. While small scale modes stay in the {\it shifted} galaxy field denoted by "D", the large scale modes are imprinted in the {\it shifted } random catalogue, denoted by "S".  The reconstructed density field is then defined as $\delta_{rec}=\delta_{d}-\delta_{s}$ that represents the sum of the two contributions of the large- and small-scale modes  \citep{PadWhiCoh}}. 


\section{Simulations}\label{sec:sim}
In this work we use two kinds of mock {\bf catalogues}. One set of approximate mock {\bf catalogues that enables us to have a sufficiently large number of realizations to test the BAO anisotropic fitting results. A second set, composed of a small number of high fidelity mocks based on N-body simulations, guarantees that the velocities are more accurate, enabling  us to test the accuracy of the reconstructed velocity field for cosmological applications. }
\subsection{Quick Particle Mesh Mocks.}\label{sec:QPM} 
Quick Particle Mesh (QPM hereafter) mocks were generated for BOSS clustering analysis. These mock {\bf catalogues} use low mass
and force resolution particle-mesh simulations employing $1280^3$ particles in a $(2560 h^{-1}$Mpc)$^3$ box run with large time steps. At select
times, the particles and their local density smoothed on $2h^{-1}$Mpc scales were dumped; these particles were then sampled (with a
density-dependent probability) to form a set of mock halos that are then populated using a halo occupation distribution \citep{QPM}.

%\sout{We use two different sets of QPM mocks for the analysis:}
%\begin{itemize}
%\sout{``Cubic mocks", which are used  in Section \ref{sec:disp} for the study of the velocity field. These mocks are also generated in the context of BOSS analysis. They reproduce CMASS galaxies in periodic cubes  with no radial or angular selection functions and 10 times higher density than a realistic BOSS sky mock. We use these cubic mocks for the velocity analysis to be able to study the accuracy of the velocity field without taking care of mask and completeness effects that will affect the displacement estimation. }
 %\sout{``Sky mocks'' , which match the observed number density of BOSS galaxies and follow the radial and angular selection functions. These mocks are required to study the anisotropic galaxy clustering and to extract conclusions applicable to current analysis of BOSS-DR12 galaxy samples.We used the version of QPM mocks that matches CMASS North Galactic Cap samples for Data Release 12 of BOSS.}
%\end{itemize}

We use ``Sky mocks'' , which match the observed number density of BOSS galaxies and follow the radial and angular selection functions. These mocks are required to study the anisotropic galaxy clustering and to extract conclusions applicable to current analysis of BOSS-DR12 galaxy samples.
We used the version of QPM mocks that matches CMASS North Galactic Cap samples for Data Release 12 of BOSS.
 %These approximate mock {\bf catalogues} contain roughly the right amount of monopole and quadrupole power, but deviate from the high resolution simulations on scales smaller than 30-50$h^{-1}$Mpc.  


\subsection{RunPB Simulations}
We use in Section \ref{sec:disp} RunPB Simulations (RunPB hereafter) \citep{white_simus} for the study of the velocity field .
The {\bf catalogues} are based on high resolution realisations of the $\Lambda -$CDM model with $\Omega_m = 0.292$ and $h = 0.69$, employing $2048^3$ particles in a periodic box of side length $1380 h^{-1} $Mpc for a total volume of $2.6 h^{-3} $Gpc$^3$. The values used at redshift $z=0.55$ for the growth factor and the power spectrum amplitude are $f=0.76$ and $\sigma_8=0.62$. The simulations were run with the TreePM code; 
the mock {\bf catalogues} are described further in \cite{whi10}. {\bf Briefly, halos were found using the friends-of-friends algorithm. We use a cut in the halo mass ($M_{halo} > 1.10^{13} \; M\odot$) which mimics the bias property of the CMASS survey}. We can do that under the assumption that most of the CMASS galaxies are Brightest Central Galaxies (BCG) ($90\%$) and so have the same velocities as the halos.

\section{Methodology}\label{sec:method}
\subsection{Anisotropic Analysis}
In this paper we follow the multipole fitting procedure described in \cite{xu12} and \cite{And13} which extracts measurements
of the isotropic dilation of the coordinates parametrized by $\alpha$ and the anisotropic warping of the coordinates parametrized by $\epsilon$. 
$\alpha$ and $\epsilon$ parametrize the geometrical distortion derived from assuming a ``wrong" cosmology when calculating the galaxy correlation function. 

The parameters $\alpha$ and $\epsilon$ are defined as
\begin{equation}
\alpha = \alpha_{\perp}^{2/3} \alpha_{||}^{1/3} \,, 
\end{equation}
and
\begin{equation}
1+ \epsilon = \left( \frac{\alpha_{||}}{\alpha_{\perp}} \right)^{1/3} \,
\end{equation}
where $\alpha_\perp$ and $\alpha_{||}$ are defined by
\begin{align}
r_{\perp} & = \alpha_{\perp} r_{\perp, {\rm obs}} 
\label{eqn:aperpdef} \\
r_{\parallel} & = \alpha_{\parallel} r_{\parallel, {\rm obs}} .
\label{eqn:apardef}
\end{align}
Here, the `obs' subscript denotes the observed coordinates. The coordinates without 'obs' subscripts
{\bf correspond to the assumed cosmology. $r_{\perp}$ and $r_{||}$ are respectively the
transverse and parallel to the line line-of-sight galaxy separations.}

The transverse shift, $\alpha_\perp$, allows us to measure $D_A(z)/r_s$,
where $D_A(z)$ is the angular diameter distance to redshift $z$ and $r_s$
is the sound horizon scale. The line-of-sight shift, $\alpha_{||}$, allows us
to measure $cz/(H(z)r_s)$ where $H(z)$ is the Hubble parameter. This is
done using
\begin{equation}
\alpha_{\perp} = \frac{D_{A} (z) r_{s,{\rm fid}}}{D^{\rm fid}_{A} r_{s}},
\end{equation}
and
\begin{equation}
\alpha_{||} = \frac{H^{\rm fid}(z) r_{s,{\rm fid}}}{H(z) r_{s}}.
\end{equation}
Note that when analyzing the mocks in the cosmology in which they are define,  $\alpha =  1$ and $\epsilon = 0$. 

\subsection{Nonlinear Models for the Correlation Function}\label{sec:NLM}

The template for the 2D nonlinear power spectrum, followed from  \cite{Fis94} reads as follows:
\begin{equation}
P(k, \mu) =(1+\beta \mu^2 )^2 F(k, \mu, \Sigma_s)P_{NL} (k, \mu),
\end{equation}
{\bf where the term $(1+\beta \mu^2)$  corresponds to the Kaiser model for large-scale redshifts distortions, which produce an anisotropic damping and $P_{NL}(k)$ is the nonlinear power spectrum.}
$F(k, \mu, \Sigma_s)$ is the streaming model for FoG  given by: 
\begin{equation}\label{eq:streamming}
F(k, \mu, \Sigma_s)=\frac{1}{(1+k^2\mu^2 \Sigma_s^2)},
\end{equation}
where $\Sigma_s$ is the streaming scale. In this work, we 
consider the de-wiggled power spectrum $P_{dw}$. To get the templates for the multipoles, we decompose the 2D power spectrum into its Legendre moments:
\begin{equation}
P_{l,t}(k)=\frac{2l+1}{2}\int_{-1}^{1}P_t(k, \mu)L_l(\mu)d\mu,
\end{equation}
which can then be transformed to configuration space using
\begin{equation}
\xi_{l,t}(r) = i^l \int \frac{k^3 d log(k)}{2 \pi^2}P_{l,t} j_l(kr),
\end{equation}
where $j_l(kr)$ is the l-th spherical Bessel function and $L_l(\mu)$ is the l-th Legendre polynomial.


\subsection{De-wiggled Template} \label{sec:dewiggled}

The de-wiggled template is a  power spectrum prescription widely used in clustering analysis \citep{xu12,And12,And13}. This phenomenological prescription takes a linear power spectrum template to which we add the nonlinear growth of structure.
The de-wiggled power spectrum is defined as:
\begin{equation}
\begin{array}{ll}
P_{dw}(k, \mu)=&[P_{lin}(k) -P_{nw}(k)] \\
&\times exp\left[ -\frac{k^2 \mu^2 \Sigma_{||}^2+k^2(1-\mu^2)\Sigma_{\perp}^2}{2}\right ] +P_{nw} ,
\end{array}
\end{equation}
{\bf where $P_{lin}(k)$ is the linear theory power spectrum and $P_{nw}(k)$ is a power spectrum without the acoustic oscillations (\cite{Eis98}). $\Sigma_{||}$ and $\Sigma_\perp$ are the radial and transverse components of the standard Gaussian damping of BAO, $\Sigma_{NL}$ :}
\begin{equation}
\Sigma_{NL}^2=(\Sigma_{||}^2+\Sigma_\perp^2)/2.
\end{equation}
 $\Sigma_{NL}$ models the degradation of signal because of nonlinear growth of structure. 


\subsubsection{Multipole Fitting}
In order to measure $\alpha$ and $\epsilon$, we define a fiducial
cosmology and then fit template multipoles (monopole and quadrupole) of the correlation function in
this fiducial cosmology to the observed data. {\bf We use the model described in \cite{xu12} to generate the templates for multipoles of the correlation function.}
This model is summarized in detail in \cite{xu12,Var14,And12,And13}.
The models we fit to our observed multipoles, $\xi_0(r)$ and
$\xi_2(r)$, are:
\begin{align}
\xi_{0}(r) &= B_0^2 \xi_{0, \rm obs}(r) + A_0(r) \nonumber, \\ 
\xi_{2}(r) &= \xi_{2, \rm obs}(r) + A_2(r),
\label{eqn:monoquadt}
\end{align}
where
\begin{equation}
A_{\ell}(r) = \frac{a_{\ell,1}}{r^2} + \frac{a_{\ell,2}}{r} + a_{\ell,3}; \,
\ell=0,2.
\label{eqn:fida}
\end{equation}
These $A_\ell(r)$ terms are used to marginalize out broadband (shape)
information through the $a_{\ell, 1}\ldots a_{\ell, 3}$ nuisance parameters. 
{\bf We use a fit he monopole and the quadrupole in a range of $50<r<200h^{-1}$Mpc, with $40$ bins of 8 $h^{-1}$ Mpc each. 
Knowing our model uses  $10$ we have finally $30$ degrees of freedom for the fit.

In order to find the best-fitting values for $\alpha$ and $\epsilon$, we 
minimize the $\chi^2$ function}
\begin{equation}
\chi^2 = (\vec{m} - \vec{d})^T C^{-1} (\vec{m}-\vec{d}),
\end{equation}
{\bf where $\vec{m}$ is the model vector and $\vec{d}$ is the vector of data.} We scale the
inverse sample covariance matrix, $C^{-1}_s$, using
\begin{equation}
C^{-1} = C^{-1}_s \frac{N_{\rm mocks} - N_{\rm bins} - 2}{N_{\rm mocks} - 1},
\end{equation}
{\bf to correct the bias in the estimate of the true inverse covariance matrix $C^{-1}$ \citep{Har07}. }

Error estimates for $\alpha$ and $\epsilon$ are obtained by walking a
grid in these two parameters to map out the
likelihood surface. Assuming that the likelihood surface is Gaussian, this allows
us to estimate $\sigma_\alpha$ and $\sigma_\epsilon$ as the standard
deviations of the marginalized 1D likelihoods of $\alpha$ and $\epsilon$
respectively. 

\section{Smoothing effect on anisotropic BAO analysis.}\label{sec:fits}


First, we study the effect of the smoothing scale in the BAO analysis described in section \ref{sec:method}. 
The results presented in this section were obtained using ``sky mocks'' described in section \ref{sec:QPM}.
{\bf We apply the reconstruction algorithm described in section \ref{sec:rec} using four different smoothing scales: 
%\sout{$R=0$
%\footnote{\sout{We must notice the R=0 means that there is no Gaussian smoothing applied, however as the density is estimated in a grid there is a intrinsic smoothing applied in addition to the Gaussian smoothing}}:,
 R=$5$, $10$, $15$ and $40 h^{-1}$Mpc.
Then, we compute the correlation function of the reconstructed {\bf catalogues}. Finally we apply the BAO fitting methodology and evaluate reconstruction performance using the fits on $\alpha$ and $\epsilon$ parameters and their respective uncertainties as a metric.}
%\sout{We include the extreme case R=0 in order to verify that the Gaussian smoothing is required for getting a good performance on reconstruction algorithm. Evidently, }
%\footnote{
\footnote{The effective smoothing scale is a convolution of the Gaussian smoothing and the grid smoothing. Hereafter we refer only to the Gaussian smoothing. We considered that the grid smoothing is not changing significantly the effective smoothing. In the 1D case, using a Gaussian smoothing equal to a grid size, the effective smoothing is ~15\% large for NGP, or ~30\% larger for CIC. The 
5 Mpc smoothing, assuming a 5 Mpc grid is really ~6 Mpc for NGP and 6.5 Mpc for CIC, which is not very different.} We summarize the details of the interpolation method used in the density estimation  in Table \ref{tab:inter}. 

%We apply the reconstruction algorithm described in section \ref{sec:rec} using five different smoothing scales: $0$\footnote{We must notice the R=0 means that there is no Gaussian smoothing applied, however as the density is estimated in a grid there is a intrinsic smoothing applied in addition to the gaussian smoothing},$5$, $10$, $15$ and $40 h^{-1}$Mpc.
%Then, we compute the correlation function of the reconstructed {\bf catalogues}. Finally we apply the BAO fitting methodology and evaluate reconstruction performance using the fits on $\alpha$ and $\epsilon$ parameters and their respective uncertainties as a metric.
%We include the extreme case R=0 in order to verify that the Gaussian smoothing is required for getting a good performance on reconstruction algorithm. Evidently, the effective smoothing scale is a convolution of the Gaussian smoothing and the grid smoothing. Hereafter we refer only to the Gaussian smoothing. We considered that the grid smoothing is not changing significantly the effective smoothing\footnote{In the 1D case, using a Gaussian smoothing equal to a grid size, the effective smoothing is ~15\% large for NGP, or ~30\% larger for CIC. The 
%5 Mpc smoothing, assuming a 5 Mpc grid is really ~6 Mpc for NGP and 6.5 Mpc for CIC.}, which is not very different. We summarize the details of the interpolation method used in the density estimation  in Table \ref{tab:inter}. 


\begin{table}
\begin{center}
\caption{ Interpolation parameters }
\label{tab:inter}
\begin{tabular}{@{}cccccccc}
\hline
Simulation & Interpolation& Box Size & Grid &Pix Size\\
&Method&($h^{-1}$Mpc)& &($h^{-1}$Mpc)\\
\hline
\\[-1.5ex]
QPM Cubic & NGP &2560 &512 &2.6 \\
QPM Sky & NGP& 3400&512& 5\\
PB Mocks & NGP& 1380 &512  & 6.6\\

\hline
\\[-1.5ex]
\end{tabular}
\end{center}
\end{table}
\subsection{Multipoles Results}
%\rr{This needs some re-writing.Also the first and second paragraphs are sometimes contradictory as to which scales are important. From Fig. 2 on the right hand side, it looks like in both cases the 10/15 Mpc/h are best at the BAO scale..this contradicts the first sentence of 5.2} %\bb{Here is just a rewriting issue. Explain to the referee that there is no contradiction with 5.2, his statement is wrong about the 10/15 smoothing scale..}

{\bf In Figure \ref{fig:meanSmooth} we show the mean multipoles from $200$ QPM reconstructed mocks with the four smoothing scales.} Upper panel is for the mean monopole and lower panel for the mean quadrupole. {\bf The shaded regions correspond to the square root of the diagonal elements of the covariance matrix. }

{ \bf For the monopole we observe two effects: 1) At large scales we find,  as expected, that the different smoothing scales affect the level of sharpening of the mean monopole.  The cases 5, 10, and 15 Mpc/h show an enhanced peak compared with the pre-reconstruction monopole.
 However the R=5 is slightly lower compared to the 10-15 smoothing scales. The R=40 is clearly decreasing the contrast in the BAO peak. 
%\sout{The R=0 case clearly shows a more smoothed peak compared to the other smoothing scales, indicating that the smoothing is required to sharpen the BAO peak.}
2) At small scales we find that the different smoothing scales affect the shape of the monopole. These scales  are not important for the fitting of the BAO feature. The differences at those scales are mostly related to the residual redshift space distortions.}%\bb{Needs to included pre-rec in the plot} 
% and eliminate 0 smoothing.}

%We find that the different smoothing scales affect the level of sharpening of the mean monopole as expected. Given the differences in amplitude, it is not obvious to determine which smoothing scale is performing better. \sout{The R=0 case clearly shows a more smoothed peak compared to the other smoothing scales, indicating that the smoothing is required to sharpen the BAO peak.}
 %The R=5 also seems slightly lower compared to the 10-15 smoothing scales. The R=40 is clearly decreasing the contrast in the BAO peak. 
%We also notice that the different smoothing scales affect the shape of the monopole at small scales, which is irrelevant for the fitting of the BAO feature. The differences at those scales are mostly related to the residual redshift distortions and are mostly absorbed by the marginalized parameters as $B_0, A_{0,\ell}$. 
% Concerning the quadrupole, Figure \ref{fig:meanSmooth} illustrates that  the typical smoothing scale of $15 $ $h^{-1}$ Mpc gives a quadrupole not completely consistent with zero. The disagreement appears worse when using a large smoothing scale where the correlation increases in the interval $50-100 h^{-1}$Mpc. Using a smaller smoothing scale reduces the negative correlation observed in the quadrupole to be in agreement with zero within the fitting range, since a perfect reconstruction would show a mean quadrupole consistent with zero (without any large-scale anisotropies). 
%
%However, it is not clear just by comparing the results in terms of correlation functions that the reconstruction is performing better with smaller smoothing scale. 
%As for BAO anisotropic fits, the important point is to have a quadrupole consistent with zero at the BAO scales, and for this scale, all smoothing lengths have the same amplitude.
%Just from the correlation function performance it is not possible to conclude if the BAO anisotropic fits will be affected. Our next task is to test if this residual anisotropy is affecting the anisotropic fits. 
%

{ \bf Concerning the quadrupole, a perfect reconstruction would show a mean quadrupole consistent with zero (without any large-scale anisotropies). Figure \ref{fig:meanSmooth} illustrates that  the typical smoothing scale of $15 $ $h^{-1}$ Mpc gives a quadrupole not completely consistent with zero. 
The disagreement appears worse when using a large smoothing scale where the correlation increases in the interval $50-100 h^{-1}$Mpc. Using a smaller smoothing scale reduces the negative correlation observed in the quadrupole to be in agreement with zero within the fitting range. }

{\bf In summary, just by comparing the results in terms of correlation functions, it is not clear that the reconstruction is performing better with any smoothing scale. Two effects affect differently the BAO anisotropic fits: 
\begin{enumerate}
\item The precision of $\alpha$ is driven by the sharpening of the BAO feature. Thus we expect, that 10-15, gives best precision on $\alpha$ followed very closely by 5, and that 40 smoothing scale increases the error on $\alpha$.
\item The precision on $\epsilon$ depends on the capability that our nuisance parameters ($B_0, A_{0,2}$) to absorb the residual quadrupole.  We can expect that a quadrupole consistent with zero is likely to give a good fit, thus we expect that 5 Mpc/h will provide best constraints on $\epsilon$, followed by 10 and 15. 
\end{enumerate}
Our next task is to test these hypotheses and check how the smoothing scales affect the anisotropic fits.}

%at the BAO scale 
% is absorbed by the marginalized parameters as $B_0, A_{0,2}$.

%the important point is to have a quadrupole consistent with zero at the BAO scales, and for this scale, all smoothing lengths have the same amplitude.
%Just from the correlation function performance it is not possible to conclude if the BAO anisotropic fits will be affected.
 %Our next task is to test if this residual anisotropy is affecting the anisotropic fits. 


%Given the differences the multipoles shapes, it is not obvious to determine which smoothing scale is performing better. and are mostly absorbed by the marginalized parameters as $B_0, A_{0,\ell}$.

\begin{figure*}
   \centering
      \includegraphics[width=3.8in]{Mean_smooth_final_bias187.pdf}\includegraphics[width=3.8in]{Mean_smooth_final_bias187zoom.pdf}    
 %  \includegraphics[width=3.8in]{Mean_smooth_final_bias187_zero.pdf}\includegraphics[width=3.8in]{Mean_smooth_final_bias187zoom.pdf}      
   \caption{ {\bf [Modified plot without zero smoothing]}. Mean of $200$ QPM mocks NGC reconstructed with different smoothing scale  $5  h^{-1}$Mpc [green] , $10 h^{-1}$Mpc [cyan],$15 h^{-1}$Mpc [magenta] and $40 h^{-1}$Mpc [blue]. The smoothing scale is correlated with the negative correlation observed in the quadrupole; smaller smoothing scale decreases the correlation observed; a $5 h^{-1}$Mpc smoothing scale erases almost completely the quadrupole. Right panel: Zoom to the monopole [top panel] and quadrupole [bottom panel] in the BAO range.}%\bb{Needs to included pre-rec}}% \bb{Needs to included pre-rec in the plot and eliminate 0 smoothing.}
   \label{fig:meanSmooth}
\end{figure*}

 
\subsection{Anisotropic Fits on the Mean Correlation Function}
%\rr{Is 5 Mpc/h really doing better in the plots? I am confused as to why the nonlinear damping parameter is higher for 15 Mpc/h than for 40. If the NL damping acts to increase the width of the correlation function bump, and at 40Mpc/h the bump is wider, how is the value of NL damping larger for 15Mpc/h. The results in Table 3 don't seem to tell the same story as the plots in Figure 2.} \bb{Here we need to add a paragraph giving an hypothesis of why we have this numbers in 15 and 40. This is a science request.}
%\sout{In order to verify that the 5 $h^{-1}$Mpc smoothing scale is performing better}

%\bb{Here we need to add a paragraph giving an hypothesis of why we have this numbers in 15 and 40. This is a science request.}

{\bf In order to determine which smoothing scale is performing better, we fit the nonlinear damping parameters $\Sigma_{\parallel, \perp}$ and the streaming parameter $\Sigma_s$ using the mean information over the mocks. In Table \ref{tab:fixpar} we summarize the results for different values of $R$. We find a minimum value for $\Sigma_{\parallel, \perp}$  for a smoothing scale of 5 $h^{-1}$Mpc, indicating that the mean correlation function is less nonlinear using this filter. When we increase the smoothing scale, the value $\Sigma_{\parallel, \perp}$ increases for 10 and 15 Mpc/h, indicating that the function is becoming more non linear. }
%\sout{When we reduce R to zero, the nonlinear damping parameter increases, indicating that the smoothing is required for getting a less nonlinear correlation function} %
%\footnote{\rr{REFEREE COMMENTS: Footnote 3 doesn't make sense.}. \bb{We need to argue why the 40 Mpc/h scale is braking down.} %\sout{extreme values,0 and} 
{\bf We note that the values we get for the $\Sigma_{\parallel, \perp}$ for the 40  case are smaller compared to 15,  this unexpected behavior is probably related with the breaking down of the assumption $\Sigma_{\parallel}=\Sigma_{\perp}$. 
At 40 Mpc/h we expect to have a poor performance of reconstruction, since we start to lose information as we are smoothing scales that are in linear regime. Therefore, applying a smoothing of 40 Mpc/h results in a very poor performance of reconstruction comparable to not doing reconstruction.  We suspect that the unexpected values obtained for the nonlinear damping are generated because we are using the fitting template for the post-reconstruction case, i.e. we are assuming that the nonlinear damping is isotropic. But this is most likely not a good approximation, since with this smoothing we are not removing most of the nonlinear evolution of the density. %because of the poor performance of reconstruction with this smoothing scale.
 Thus, it would be more accurate to do the fitting with both damping parameters free instead . }%, but in our methodology we are forcing them to be identical.
%We note that the larger values we get for the $\Sigma_{\parallel, \perp}$ for the  40 case,  are probably related with the breaking down of the assumption $\Sigma_{\parallel}=\Sigma_{\perp}$.}. 
%  
  {\bf In order to test that the assumption $\Sigma_{\parallel}=\Sigma_\perp}$ is breaking down for R=40, we performed for all cases a fit without this assumption (see bottom panel of Table \ref{tab:fixpar}). For 40 Mpc/h we get a $\chi^2/d.o.f$  higher  when $\Sigma_{\parallel}$ and $\Sigma_\perp}$ can vary. However for the cases R=5,10 15, the $\chi^2/d.o.f$ is much higher when we asume $\Sigma_{\parallel}=\Sigma_\perp}$.} 

We also notice that the $\beta$ value fitted is the smallest for $5h^{-1}$Mpc, indicating that the correction for the Kaiser effect is less important for a smaller smoothing scale. Also interesting to note is that we get the higher $\chi^2/d.o.f$  for 5 $h^{-1}$Mpc smoothing scale. 
In the case of the streaming parameter $\Sigma_s$, which is related to the Fingers-of-God (FOG) effect,  we do not expect to find any improvement (to find any change) in the best fitting value for this parameter, since reconstruction does not take care of virial velocities.  

\begin{table}
\begin{center}
\caption{ {\bf [Modified Table without zero smoothing]}. Values for the fixed parameters fitted to the mean of 200 QPM mocks varying the smoothing scale of  reconstruction. }
\label{tab:fixpar}
\begin{tabular}{@{}ccccccc}
\hline
R & $\Sigma_\parallel= \Sigma_\perp$ & $\Sigma_s$& $\chi^2/d.o.f$ & $B_0$ & $\beta$\\
($h^{-1}$Mpc)&($h^{-1}$Mpc)&($h^{-1}$Mpc)& &&\\
\hline
\\[-1.5ex]
%0 & 6.8 &8.1 &14.4/30 &0.73 &-0.05}\\
5 & 4.9 & 0.0 &18.4/30 & 0.98&-0.06\\
10 &5.7& 0.0 &9.4/30   & 1.01&-0.12\\
15&6.5 & 0.0 &14.3/30&  1.28&-0.11\\
40& 5.9&-6.0 & 11.3/30 &1.31&0.29\\
\hline
R & $\Sigma_\parallel$&$\Sigma_\perp$ & $\Sigma_{NL}$&  $\chi^2/d.o.f$ & $B_0$ & $\beta$\\
\hline
5&4.8& 5.6 &5.2&7.0/30 &0.9 &0.01\\
10&5.9& 1.5 &4.3&8.2/30 &1.0 &-0.13\\
15&6.9& 3.6 &5.5&10.3/30 &1.2& -0.10\\
40&5.6 &8.8&7.3&14.7/30 &1.3 &0.35\\
\hline
%\hline
%R & $\Sigma_\parallel$&$\Sigma_\perp$ & $\Sigma_s$&$\chi^2/d.o.f$  & $\beta$\\
%\hline
%0 &  &&&&\\
%40 &  &&&&\\
\hline
%PTHALOS\\
%\hline
%15 & 3.0 &1.4 &-&-\\
% \hline
\\[-1.5ex]
\end{tabular}
\end{center}
\end{table}

\subsection{Anisotropic Fits Results}\label{sec:anisofits}
%\rr{-It seems strange that the 15Mp/h smoothing gives different results from the other cases. Is exactly the same data used? Also I am confused with the last sentence in the first paragraph. The 10 Mpc/h shows 0.5 which is less than 0.8.}

{\bf In Figure \ref{fig:MeanParSmooth} we show the results from fitting  200 QPM mocks reconstructed using the four smoothing scales.} We show the mean value from the best fits for BAO-related parameters $\alpha$[top panel], $\epsilon$[bottom panel].  We also show in Figure \ref{fig:MeanParSmooth2}  results for $\beta$[bottom panel], and the $\chi^2$  [top panel] results for the fits.  The dotted line indicates the expected values from the mocks. The quantitative fitting results are summarised in Table \ref{tab:fits} for the best fits in anisotropic BAO analysis.

The accuracy in the $\alpha$  value is very similar between $5$ and $15 h^{-1}$Mpc but visibly degrades when going to higher smoothing scales. 
The smaller dispersion for $\alpha$ is for 10-15 $h^{-1}$Mpc; however, the 15 $h^{-1}$Mpc is significantly biased (5.3 $\sigma$), {\bf thus, 10$h^{-1}$Mpc is the best option if we considered only $\alpha$.} \bb{ In order to understand the significantly larger bias found in 15 Mpc/h case we decide to check the individual fits and compared to 10 Mpc/h case. We show in Fig [missing] %\ref{fig:dispersionplots15vs10}
 the distribution of the different parameters as a sanity check to try to find the source of the observed bias.}

For $\epsilon$, the least significant bias ($b_\epsilon/\sigma_\epsilon$ lower) is for 5 $h^{-1}$Mpc smoothing scale. {\bf Considering $\alpha$ and $\epsilon$ simultaneously, the best option is 5 $h^{-1}$Mpc which gives the less significant bias with smaller dispersion (0.8$\sigma$ in $\alpha$ and $0.9\sigma$ in $\epsilon$ ).} %\sout{the smaller dispersion is for zero smoothing; however, the bias for this case is the largest (3.2$\sigma$).} 

We find maximal variations in the mean value for best fit parameters  $\sim$0.5\% for $\alpha$ and 0.3\% for $\epsilon$, producing $\Delta D_A , \Delta H\sim 0.5$\%. 
In the case of  $\beta$, the precision seems to be very similar for the $5$ and $15 h^{-1}$Mpc smoothing scales and slightly lower for the 40 $h^{-1}$Mpc. The accuracy is also similar for $5$ and $15h^{-1}$ smoothing scales and clearly degrades when using a higher smoothing scale. The $\chi^2/d.o.f$ values are very similar between the different smoothing scales explored. \footnote{The values  of the $\chi^2\sim$0.8  are similar to those obtained with the reconstruction implementation used in previous analysis. We add more discussion about the results using different implementations in Appendix \ref{ap:imp}.}



{\bf Figure \ref{fig:errors} presents the distributions of the uncertainties for $\alpha$ and $\epsilon$  parameters for different smoothing scales and the quantitative fitting results for the uncertainties are summarised in Table \ref{tab:err}. We can see that the smoothing scale strongly affects the error distributions. and that the error bars decrease using  5 $h^{-1}$Mpc smoothing scale. The mean error  is reduced by 13\% for $\alpha$ and 24\% for $\epsilon$ when passing from 15 to 5 $h^{-1}$Mpc.}

 
{\bf In this section, we have shown how the smoothing scale affects the anisotropic clustering results and we found that  the smaller bias and error bars are obtained using a smoothing scale of  $5 h^{-1}$Mpc.  In order to associate a systematic error, we used the scale $15 h^{-1}$Mpc as the fiducial smoothing.} We observe that varying the smoothing length from $15$ to $5h^{-1}$Mpc generates a $\Delta \alpha=0.005$ and $\Delta \epsilon=0.001$ (Table \ref{tab:fits}). Concerning the errors, the variation observed is $\Delta \sigma_\alpha=0.002$ and $\Delta \sigma_\epsilon=0.012$. Expressing these variations in the best fits and their uncertainties to the final measurements of the angular diameter distance and Hubble parameter, we get variations of $\Delta \sigma_{D_A}\sim$ 40\% and $\Delta \sigma_H\sim$33 \%. 
 

\begin{figure}
   \centering     
   \includegraphics[width=3.7in]{BestFitsSmoothingResults_alphaepsilon_bias187.pdf}%{BestFitsSmoothingResults_alphaepsilon_bias187zero.pdf}
    \caption{ {\bf [Modified plot without zero smoothing]}. Mean of best fits for $\alpha$ and $\epsilon$ for $200$ QPM mocks NGC analysed with different smoothing scales. The error bars are given by the standard deviation from $200$ realisations. For $\alpha$ the smaller dispersion is for 10-15 $h^{-1}$Mpc; however, the 15 $Mpc/h$ is significantly biased (5.3 $\sigma$). The best is 5 $h^{-1}$Mpc that has less significant bias with small dispersion (0.8$\sigma$). For $\epsilon$, the less significant bias ($b_\epsilon/\sigma_\epsilon$ lower) is for 5 $h^{-1}$Mpc smoothing scale given their small bias and dispersion. }
   \label{fig:MeanParSmooth}
\end{figure}
\begin{figure}
   \centering     
      \includegraphics[width=3.7in]{BestFitsSmoothingResults_chi2_bias187.pdf}
     \caption{ {\bf [Modified plot without zero smoothing]}. Mean of best fits for $\beta$ and $\chi^2/d.o.f.$ for $200$ QPM mocks analysed with different smoothing scales. The error bars are given by the standard deviation from $200$ realisations. The 5,10 $h^{-1}$ Mpc smoothing scale gives similar RMS and bias for linear redshift distortion parameter $\beta$ but slightly more bias for larger smoothing. Even though $\beta$ is a nuisance parameter in BAO analysis, it is interesting to observe the value fitted as it indicates the level at which the redshift corrections are using the right value of the velocity field. The $\chi^2/d.o.f$ values are very similar between the different smoothing scales explored. }
   \label{fig:MeanParSmooth2}
\end{figure}



\begin{table}
\begin{center}
\caption{{\bf [Modified Table without zero smoothing]}. Best fits for $\alpha$ and $\epsilon$. Mean, RMS from 200 reconstructed QPM mocks. } \label{tab:fits}
\begin{tabular}{@{}lcccccccccc}
\hline
$R$&
$\widetilde{\alpha}$&RMS&$\frac{b_\alpha}{\sigma_\alpha}$&
$\widetilde{\epsilon}$&RMS&$\frac{b_\epsilon}{\sigma_\epsilon}$&
$\widetilde{\beta}$&RMS\\\\

\hline
%0 &    0.9976 & 0.0157 & 2.2 &0.0023 & 0.0106 & 3.2 &-0.062 & 0.085\\
5 &      0.9992 &     0.0136 &        0.8 &     0.0007 &     0.0109 &        0.9
 &    -0.035 &     0.090 \\
10 &      1.0004 &     0.0128 &        0.5 &     0.0024 &     0.0142 & 
       2.4 &    -0.025 &     0.088\\
15 &      1.0048 &     0.0128 &        5.3 &     0.0021 &     0.0169 & 
       1.7 &    -0.019 &     0.085 \\
40 &      1.0002 &     0.0147 &        0.2 &    -0.0048 &     0.0224 & 
       3.0&     0.102 &     0.077 \\
\hline
\\[-1.5ex]
\end{tabular}
\end{center}
\end{table}

\begin{table}
\begin{center}
\caption{ {\bf [Modified Table without zero smoothing]}. Uncertainties in $\alpha$ and $\epsilon$ parameters. Median, 16 and 84 percentiles of the uncertainties distributions from 200 reconstructed QPM mocks.} 
\label{tab:err}
\begin{tabular}{@{}lcccccccccc}
\hline
$\Sigma$&
$\widetilde{\sigma_\alpha}$& $\Delta \sigma_\alpha$\%&
$\widetilde{\sigma_\epsilon}$&$\Delta \sigma_\epsilon$ \% \\
\hline
$5$&
$0.0136^{+0.0021}_{-0.0019}$&-9.9&
$0.0118^{+0.0028}_{-0.0017}$&-45.9\\
\\[-1.5ex]

$10$&
$0.0142^{+0.0030}_{-0.0019}$&-5.9&
$0.0167^{+0.0040}_{-0.0024}$&-23.4\\
\\[-1.5ex]
    15&
$0.0151^{+0.0030}_{-0.0023}$&-&
$0.0218^{+0.0062}_{-0.0039}$&-\\
\\[-1.5ex]

$40$&
$0.0150^{+0.0042}_{-0.0023}$&$-0.7$&
$0.0233^{+0.0080}_{-0.0041}$&6.9\\
\\[-1.5ex]

    
 \hline
\\[-1.5ex]
\end{tabular}
\end{center}
\end{table}


\begin{figure}
   \centering     
   \includegraphics[width=1.6in]{Hist_SigmaAlpha_smooth200v2.pdf}
   \includegraphics[width=1.6in]{Hist_SigmaEpsilon_smooth200v2.pdf}
  \caption{  {\bf [Modified plot without shading]} %\rr{Figure 5 would be better unshaded, it is difficult to see the width of the histograms but not crucial}
   Histograms of uncertainties in $\alpha$ and $\epsilon$ measured for the individual reconstructed mocks for different smoothing scales, 5 (green), 10 (cyan), 15(red) and 40 (blue). The distributions depend strongly on the smoothing scale used in the reconstruction. }
   \label{fig:errors}
\end{figure}

\subsection{Dependence on Reconstruction Implementation}
%\rr{the last paragraph needs re-writing.}

 In Appendix \ref{ap:imp} we show that  the results obtained in this work for the best smoothing scale, in terms of anisotropic fits performance, are independent of the particular implementation of reconstruction algorithm. We compare our implementation of the reconstruction algorithm to the method implemented by \cite{Pad12}.
 We compare results in terms of the multipoles. Figure \ref{fig:mean_smooth_bias21} shows the mean multipoles for the different implementations using three different smoothing lengths, 5, 10, and 15 $h^{-1}$ Mpc. {\bf We observe that the monopole behaviour is consistent between different implementations in the fitting range.} The differences observed are only important at scales smaller than 20 $h^{-1}$ Mpc.  The amplitude of the quadrupole between different implementations is significantly different. {\bf RP implementation shows a positive quadrupole which means that the reconstruction implementation is over-correcting the anisotropy. 
 %The quadrupole for RP shows a positive amplitud shown that the reconstruction implementation overcorrects the anisotropy,  \sout{is pretty similar} \sout{In the case of the quadrupole,}
 On the other hand, our implementation of reconstruction shows a negative quadrupole, which means that our implementation is under-correcting the anisotropy; }however, both quadrupoles are very similar in shape. Differences in the quadrupole are generated by two effects, redshift distortions correction and effects of the angular and radial selection functions, which are implemented in slightly different ways. Further exploration and quantification of these two contributions that generates differences in the quadrupole amplitude are treated in Vargas-Maga\~na et al (in prep).



{\bf We fitted the multipoles post-reconstruction from both implementations and compared the results. The results are completely consistent between both implementations, the differences between the mean of  the two implementations is  ~0.1\% for $\alpha$ and $\epsilon$. }Also the RMS of the best fits are similar at 0.1\% in both quantities. Concerning the errors, the dispersion of the distributions are also very similar; however, {\bf there is a} systematic larger error in RP implementation compared to RV in $\alpha$ and $\epsilon$. However the same trends are observed in both implementations; the error in $\epsilon$ is monotonically decreasing as we apply a smaller smoothing scale.  In the case of $\alpha$ the errors we get with 5 and 10 $h^{-1}$ Mpc smoothing scale are very similar, but smaller than using the 15 $h^{-1}$ Mpc that is regularly applied in BAO analysis.

\section{Smoothing effect on accuracy of displacement field estimation.}\label{sec:disp}
 In this section, we explore the effect of the smoothing scale on the reconstructed displacement field  to figure out the origin of the improvement  observed in the post-reconstruction anisotropic clustering.  In particular , we investigate if 
the improvement is related to the better estimation of the displacement field when we reduce the smoothing scale applied in the reconstruction algorithm.

{\bf Moreover, }the peculiar velocity of galaxies is a valuable quantity in cosmology since it contains complementary information to that enclosed in the galaxies position.
In the literature, there are many strategies with different approximations to obtain the velocity field.
Reconstruction provides the simplest approach to get {\bf a model dependent  reliable velocity field at large scales}. For reconstruction, the velocity field is obtained using the well-known Zeldovich approximation, in which the displacement field is given by the gradient of the gravitational potential at $\vec{q}$.
The range of applicability of this method is limited to very large scales as it fails to describe the dynamics of a nonlinear field \citep{Kit12}. {\bf Even though it has a limited range of applicability, the velocity field from reconstruction provides a direct method to constrain gravitational model comparing with velocity measurements}% \sout{could be used for many aspects of cosmology}.}

In this section we analyse the accuracy of the velocity field derived from reconstruction and then the effect of the smoothing length  on the estimated velocity field. Instead of working with velocity field we transformed the velocity to displacements using the continuity equation:
\begin{equation}
\Psi_i =v_i/f(z)H(z),
\end{equation}
were $f$ is the growth factor at redshift of the snapshot and $H(z)$ is the Hubble parameter. 

First we evaluate the quality of the recovered displacement field from reconstruction compared with simulations. {\bf This test is important for validating the use of displacement field for other cosmological applications such as the measurement of the kSZ effect \citep{Scha16,ksZPlanck,ksZ3}.
%Second, we study how the statistical properties of the displacements are affected by smoothing length. We also compare the empirical results with the theoretical predictions using linear theory.
% {\bf The purpose of this section are: first, to show the limits of validity of the linear theory, i. e the requirement of simulations for exploring the small scales, and second, the agreement of the simulations in the linear regime with the theoretical predictions.}
Second, we explore the similarity between the simulated and reconstructed displacement fields at different scales, using the correlation coefficient for different smoothing scales. % {\bf The results of this section are relevant when the optimal scale is function of the displacement field accuracy and not the reconstruction performance for BAO purposes.}
Finally, we present an estimate of the uncertainties associated with the reconstructed displacements for individual galaxies and the bias of the displacement estimations with respect to the true displacements as a function of the smoothing length.}

%For this section we used a different set of mock {\bf catalogues} 
%\sout{We used two sets of mock {\bf catalogues} for the different tests; the QPM cubic real-space mocks, \sout{the sky-QPM mocks,} and} 
%the cubic PBrun real space mocks. 
%\sout{We use QPM mocks because the fitting relies in these mocks {\bf catalogues} and we want to understand if we can explain the improvement with smoothing scale from a better estimate of the displacement field. }\sout{The main purpose of using different sets of simulations is: 1) The different cubic simulations (QPM, PBRun) are intrinsically different, so we do not expect them to give us the same answer necessarily}. 
%We use \sout{also the} PBRun mocks because they have more accurate velocities; even if we do not have them in enough number for studying the statistical properties of the fits we wanted to extend the results for surveys with samples that are not BOSS-like, i.e coming from different halo masses. \sout{they do not have realistic properties; 2) Testing with sky mocks is natural as the fits are done with these mocks, and we want to understand if we can explain the improvement with smoothing scale from a better estimate of the displacement field.

{\bf For this section we use a different set of mock {\bf catalogues}: the cubic PBrun real space mocks. 
We use PBRun mocks because they are expected to have more accurate velocities; even if we do not have a large number of these mocks to study the statistical properties for BAO fits, we have enough galaxies in each of them to accurately compare the individual velocities with the reconstructed field.}%\sout{reconstruct we want to extend our results to surveys with samples that are not BOSS-like, e.g., coming from different halo masses}}
%\sout{they do not have realistic properties; 2) Testing with sky mocks is natural as the fits are done with these mocks, and we want to understand if we can explain the improvement with smoothing scale from a better estimate of the displacement field. 
%\rr{choose one of the two}
%We use the sky-QPM mocks as  we want to understand if we can explain the improvement with smoothing scale from a better estimate of the displacement field. We use the cubic PBrun real space mocks. The PBRun mocks have more accurate velocities; however, they do not have realistic properties;}
\footnote{The ideal set of mocks for testing the displacement field accuracy would be high fidelity mocks with reliable velocities with the properties of the survey; however, we only have available high fidelity mocks without the mask of the simulations (PBrun mocks).}.

\subsection{Reconstructed Displacement Field}
%\rr{I am not sure what this subsection is supposed to show, or the benefit of this test. You are showing the differences between fields smoothed on different scales. Does this serve any purpose. I am not sure of the goal here or what the result tells us. I would suggest removing this sub-section and Fig.6.}

 {\bf The purpose of this subsection is  to show that reconstruction is providing a reliable estimate of the true displacement field but it is limited to reproduce the large scales.  We analyze the quality of the reconstructed displacement field as compared to the true displacement field.}
%\sout{We use for this section the QPM mocks in cubic boxes. The QPM cubic boxes have 10 times the number density of the sky mocks in real space.  We chose this set of mocks for this test because we wanted to avoid any degradation of reconstruction performance related to the mask or completeness of a realistic sky mock or redshift distortions. }
%\rr{ CHECK Cloud-In-Cell (CIC)} 
For analyzing the similarity between the two displacement fields, we estimate the displacement field from the particles using a assignment in a grid of $256^3$ pixels of size (10 $h^{-1}$ Mpc)$^3$. In Figure \ref{fig:velfield_smooth} we show the x-component of the displacement field, $\Psi_x$, from reconstruction (top panels) and the true corresponding displacement from simulations (bottom panels). We just show one component of the vector field as  the other two components are completely similar. The $\Psi_x$ is a 3-D scalar field; for the illustration,  we show average three pixels in one direction and we show the other two directions of the scalar field. 
Top panels show the reconstructed field for two smoothing scales, bottom panels the simulated field for the same scales.
 %\sout{The plots are obtained by subtracting recursively the $\Psi_x$ field between two smoothing scales using a Gaussian filter with smoothing scale $R_n=(2^{n}\times $(10$h^{-1}$ Mpc)) and $R_{n-1}=(2^{n-1}\times$ (10$h^{-1}$ Mpc)). }
%\begin{equation}
%\sout{\Delta \Psi_x= \Psi_x * W_G(k,R_{n}) -\Psi_x * W_G(k, R_{n-1})}
%\end{equation}
%\sout{Each panel shows $\Delta \Psi$, the difference between two smoothed fields, i.e. the structures between the two corresponding scales for $n=1,..,5$. The scales shown in the figure are expressed in comoving coordinates. From left to right, 160-320 $h^{-1}$ Mpc, 80-16 $h^{-1}$ Mpc, and 40-80 $h^{-1}$ Mpc, 20-40 $h^{-1}$ Mpc, and 10-20 $h^{-1}$ Mpc, respectively. We show how, between scales from 40 $h^{-1}$ Mpc to 320 $h^{-1}$ Mpc,}
 The plot shows the reconstructed displacement field reproduces the simulation displacement field at scales of X, demonstrating the accuracy of the reconstructed displacement field. However, we observe that, at smaller scales (smoothing X $h^{-1}$ Mpc), the reconstructed displacement field shows less structures compared with the mock {\bf catalogue }displacement field.  
\begin{figure*}
   \centering     
    \includegraphics[width=6.8in]{Map_Displacement_Velocity_smoothed_10Mpc}%{dispsim_vs_disprec_20.png}%{velocities3.pdf}
  \caption{  {\bf [New figure] Comparison of the displacement field from a PBrun simulation [left] and from reconstruction [right]. 
%  \sout{Each panel shows $\Psi$, the difference between two smoothed fields, i.e. the structures between the two corresponding scales for $n=1,..,5$.%The plots are obtained by subtracting the smoothed $\Psi_x$ field using a Gaussian filter between two smoothing scales.
%  The scales shown in the figure are in comoving coordinates, from left to right, 160-320 $h^{-1}$ Mpc, 80-160$h^{-1}$ Mpc, and 40-80$h^{-1}$ Mpc and  20-40$h^{-1}$ Mpc respectively. Between scales from 40 to 320 $h^{-1}$ Mpc,} 
The reconstructed field reproduces the structure of the true velocity field, demonstrating the accuracy of the reconstructed displacement field.} \label{fig:velfield_smooth}}%\bb{This plot will be replaced by a simpler version.}}  
\end{figure*}
%\subsection{RMS Displacement for Different Smoothing Scales.}
%\comment{Section Removed}
%\rr{I don't understand the point of comparing the true displacements to a smoothed version. The greater the smoothing length the smaller the amplitude of the density perturbation (both linear and non-linear parts) and the smaller the inferred displacement. Figure 7, 10 11 and 12 only seem to be telling me that if I smooth something with a Gaussian kernel then it's amplitude will decrease.}
%
%We study now the effect of smoothing in terms of the RMS of the displacement distributions. We performed reconstruction using different smoothing lengths, and we study the displacement distributions of the different components of the velocity. We project the displacements vectors in spherical coordinates, $dr, d\theta, d\phi$. We show in Figure \ref{fig:histcubemocks} the displacement distributions of the radial component; the other two components are completely similar. The different colors of the lines refer to the distributions generated using different smoothing lengths for reconstruction: R=5, 10, 15, 20 and 40 Mpc/h. We clearly observe the dependency of the RMS of the distributions with the smoothing length $R$. In black we show the true displacement distribution. The smaller the smoothing scale, the better the match to the simulation distribution of the displacements.
%
%\begin{figure}
%   \centering    
%	\includegraphics[width=2.5in]{Histo_1D_Displacements_reconstruction_Real_simu1.pdf}
%	 \caption{Displacement distributions of one of the components of the reconstructed displacement field generated using different smoothing length for reconstruction R=5, 10, 15, 20 and 40 Mpc/h. The RMS of the distribution varies as a function of  the smoothing lengths $R$. In black we show the true displacement distributions from simulations. The smaller the smoothing scale is the better we match to the simulation distribution of the displacements.}
%	    	\label{fig:histcubemocks}
%\end{figure}
%
%Additionally, we would like to compare the empirical results with some theoretical predictions. 
%Following the calculus from \cite{Gramann1998}, the variance of velocity fluctuation on a given scale $r$ can be expressed as
%\begin{equation}
%\left<v^2(R)\right> = \int V^2(k)W^2(kR)\frac{dk}{k},
%\end{equation}
%where $W^2(kR)$ is the Fourier Transform of a window function and $V^2(k)$ gives the contribution to the velocity dispersion per unit interval in $\ln (k)$. For a Gaussian window function, which corresponds to our smoothing function, the RMS velocity of the matter is given by
%\begin{equation}
%v_{rms}^2(R) = \int V^2(k)\exp(-R^2k^2) \frac{dk}{k}.
%\end{equation}
%Within the linear approximation, and considering no vorticity, the function $V^2(k)$ can be determined as:
%\begin{equation}
%V^2(k) = \frac{1}{2\pi^2}f^2(\Omega_0,z)H_0^2kP(k).
%\end{equation}
%Under these assumptions we finally obtain the theoretical linear approximation of the displacements RMS by \rr{do not have the correct units Also exp, log etc. should be in roman so change these i.e. use $\exp{x}$}
%\begin{equation}
%\Delta_{rms}(R) = \frac{\sqrt{v_{rms}^2(R)}}{H_0f(\Omega_0,z)} = \left( \frac{1}{2\pi^2}\int kP(k) \exp(-R^2k^2) \frac{dk}{k}\right)^{1/2}.
%\end{equation}
%We show, in Figure \ref{fig:Comparaison_rms_th_mariana}, the comparison between the theoretical $\Delta_{rms}(R)$ in one dimension for $z=0.57$ and the $\Delta_{rms}(R)$ that we measure with the reconstruction for different smoothing radii. The 1D value is simply obtained by dividing by a factor $\sqrt{3}$ the 3D $\Delta_{rms}(R)$ under the assumption of isotropy. The displacements from reconstruction are in good agreement with the theoretical predictions for the RMS displacement in the linear regime. It is expected that at very small scales, the linear regime breaks down as observed in the Figure \ref{fig:Comparaison_rms_th_mariana}. 
%\begin{figure}
%\begin{center}
%\includegraphics[width=10cm]{QPMD_Displacements_Vs_radius_z=0_57.pdf}
%\caption{Comparison between theoretical linear RMS of the displacements and the RMS of the reconstruction obtained in one dimension considering different smoothing scales $R$. We find that a dispersion of velocity is well described by the linear approximation for different smoothing scales.  We find a discrepancy at very low smoothing scale as expected because this expression is valid only in the linear regime. The error bars represent the $3\sigma$ RMS obtain using thirty simulations.}
%\label{fig:Comparaison_rms_th_mariana}
%\end{center}
%\end{figure}

\subsection{Accuracy of Displacement Field Estimation}
%\rr{I don't really understand this section. Is it saying that on large scales the smoothing length doesn't matter so much but as you approach the scale of the smoothing length you see changes between distributions smoothed on different scales.}

To quantify the accuracy of  displacement reconstruction, we compute the correlation coefficient between the displacement from the mocks and the displacement from reconstruction. The correlation is defined as:
\begin{equation}
c(k)=\frac{<\Psi_{sim} \cdot \Psi_{rec}>}{\sqrt{P_{\Psi,sim}(k) P_{\Psi,rec}(k)}}
\end{equation}
where $P_{\Psi,rec}=<\Psi_{rec} \cdot \Psi_{rec}>$ is the power spectrum of norm of displacement field vectors and $P_{\Psi,sim}=<\Psi_{sim} \cdot \Psi_{sim}>$ is the analogous for simulations. For computing this displacement field we use the displacement vector from the galaxies, and we use a Cloud-In-Cells assignment in a grid $512^3 $. We tested the effect of using a different grid size in the appendix. In Figure \ref{fig:crossvel_smooth} we show the coefficient of cross-correlation for different smoothing scales $5,15, 40$$h^{-1}$ Mpc. {\bf The grid size and interpolation used is specified in Table 2. }%Correlation equal to one means both fields are completely correlated, as we moved the smoothing scale this correlation increases at smaller scales, but after certain scale we do not recover more information.
 We observe that the coefficient of cross-correlation improves (i.e. gets closer to 1 for larger values of k) when we decrease the smoothing scale; {\bf Correlation equal to one means both fields are completely correlated. With the usual 15 Mpc/h smoothing scale, the correlation between fields drops at k=X, as we decrease the smoothing scale this correlation increases at smaller scales. Thus we are recovering more information from the density field and we are getting a displacement field that is in agreement with the true displacement at larger $k$ thus at smaller scales .} This result verifies the hypothesis that the velocities recovered in reconstruction are correlated  with the true velocities to larger $k$ (i.e at smaller scales) when they are computed using a smaller smoothing scale. If we take as a reference point a cross-correlation coefficient of $c(k)=0.8$, the larger $k$ value we get using a $40h^{-1}$Mpc  smoothing scale is $\sim 10^{-2}$ h Mpc$^{-1}$ which corresponds to a scale $\sim62 Mpc/h$. This scale indicates up to which scale the displacement field we recovered reproduces the true displacement. For  $15h^{-1}Mpc$  smoothing scale, the largest k we get is  $\sim 2\times10^{-2} hMpc^{-1} $(20$h^{-1}$ Mpc); and using $5h^{-1}$Mpc  smoothing scale, we reach a $k$ maximal of  $\sim 4\times10^{-2} hMpc^{-1} $(15$h^{-1}$ Mpc). 

\begin{figure}
   \centering    
        \includegraphics[width=3.3in]{CrossCorVelSimRec_NGP_smooth2.pdf}
  \caption{Coefficient of Cross-correlation between Velocity Field from Simulations and Velocity Field from Reconstruction for different smoothing scales for PBRun \sout{Cubic QPM} mocks. In green 5 $h^{-1}$ Mpc , in magenta 15 $h^{-1}$ Mpc and in blue 40 $h^{-1}$ Mpc. We observe the coefficient of cross-correlation improves (i.e. gets closer to 1 for larger values of k) when we decrease the smoothing scale.The velocities recovered in reconstruction are correlated  with the true velocities to larger $k$ (i.e at smaller scales) when they are computed using the smaller smoothing scale of 5 $h^{-1}$ Mpc. \bb{This plot need to be generated with the  PBrun mocks.}}
   \label{fig:crossvel_smooth}
\end{figure}
\subsection{Error and Bias of Reconstructed Displacements}
%\rr{Again I think that this section can be removed including the figures it relates to as I am not sure that it tells us anything.}

Up to now we have been using the values of the displacement field in pixels. Now we are interested in comparing the individual values of the displacement for each galaxy to evaluate their agreement to the simulations. We expect only be correct on the linear component of the velocity field. We are also interested in associating an error to those velocities; %we will be interested in 
this is interesting if we use those velocities for inferring cosmological information for other applications than BAO.

We study the dispersion between true and reconstructed displacements.  We estimate the 2D-histograms mock-by-mock for different smoothing scales. %  \sout{for 10 mocks.For this test}
 We used the PBrun cubic mocks. %\sout{three sets of mocks QPM cubic, QPM, sky, } 
%\sout{In Figure \ref{fig:hist2dcube} we show the Cubic QPM mocks histograms.  } %\sout{the QPM sky-mocks are shown in Figure \ref{fig:hist2dsky_RD}.}
 In Figure \ref{fig:hist2dPBrun} we show the same 2D-histograms for PBrun Cubic mocks. The dotted black line indicates the 1-1 relation. The solid line comes from a 2D-Gaussian fitting to the 2D histogram; it represents the angle between the major axis and the ordinate axis. This angle cannot be interpreted as the bias of the reconstructed displacements compared with the true displacements, but it provides an illustration of the effect. In the Section  \ref{biasrec} we describe the methodology we follow to characterise the bias and noise in the displacement estimation and we present the results in \ref{biasrecres}. The derivation of the equations is presented in Appendix \ref{ap:biasnoise}. 

%
%\begin{figure*}
%   \centering    
%\includegraphics[width=1.35in]{Paper_Gauss2Dfit_R=0_QPMcube.pdf}\includegraphics[width=1.35in]{Gauss2Dfit_R=5_QPMD_simu1.pdf} \includegraphics[width=1.35in]{Gauss2Dfit_R=10_QPMD_simu1.pdf}\includegraphics[width=1.35in]{Gauss2Dfit_R=15_QPMD_simu1.pdf}\includegraphics[width=1.35in]{Gauss2Dfit_R=40_QPMD_simu1.pdf}
%	 \caption{Scatter plots between true and reconstructed displacements from different smoothing scales, from left to right R=0,5,10,15,40$h^{-1}$ Mpc. The mocks used in this test were in real space. The dashed black line indicates the 1-1 relation.
%	 The solid line comes from fitting a 2D-Gaussian to the 2D histogram; it represents the angle between the major axis and the ordinate axis. 
%	  This angle does not  indicate the bias of the reconstructed displacements compared with the true displacements but provides an illustration of the effect.	  
%	  The results of the bias and noise are presented in the Table \ref{tab:noise_bias_norsd}. The quality factor and coefficient of correlation indicate that the best result is obtained using the  5 $h^{-1}$ Mpc smoothing scale, showing the higher correlation coefficient and the lower quality factor.}
%   	\label{fig:hist2dcube}
%\end{figure*}
\begin{figure*}
   \centering
%   	\includegraphics[width=1.4in]{Paper_Gauss2Dfit_R=0_mcut_1_0e13.pdf}
\includegraphics[width=1.8in]{Paper_Gauss2Dfit_R=5_mcut_1_0e13.pdf}\includegraphics[width=1.8in]{Paper_Gauss2Dfit_R=10_mcut_1_0e13.pdf}\includegraphics[width=1.8in]{Paper_Gauss2Dfit_R=15_mcut_1_0e13.pdf}\includegraphics[width=1.8in]{Paper_Gauss2Dfit_R=40_mcut_1_0e13.pdf}
	  \caption{PBrun mocks. Scatter plots between true and reconstructed displacements from different smoothing scales, from left to right R=5,10,15,40 $h^{-1}$ Mpc. The mocks used in this test were in real space. The dashed white line indicates the 1-1 relation.
	 The solid line comes from fitting a 2D-Gaussian to the 2D histogram; it represents the angle between the major axis and the ordinate axis. This angle does not  indicate the bias of the reconstructed displacements compared with the true displacements but provides an illustration of the effect. 
	  The best result is obtained for the 5 $h^{-1}$ Mpc according to our quantitative results shown in Table \ref{tab:noise_bias_pbrun}. These mocks have more realistic velocities compared to QPM mocks.}
	    	\label{fig:hist2dPBrun}
\end{figure*}

%{\bf [Scatter plots between true and reconstructed displacements from different smoothing scale for QPM  eliminated]}

%\begin{figure*}
%   \centering    
%   \includegraphics[width=1.35in]{Gauss2Dfit_R=0_QPMDsky_simu1_julydr3.pdf} \includegraphics[width=1.35in]{Gauss2Dfit_R=5_QPMDsky_simu1_julydr3.pdf} \includegraphics[width=1.35in]{Gauss2Dfit_R=10_QPMDsky_simu1_julydr3.pdf}\includegraphics[width=1.35in]{Gauss2Dfit_R=15_QPMDsky_simu1_julydr3.pdf}\includegraphics[width=1.35in]{Gauss2Dfit_R=40_QPMDsky_simu1_julydr3.pdf}
%	  \caption{\rr{eliminated}\sout{Sky mocks in redshift space. Scatter plots between true and reconstructed displacements from different smoothing scales, from left to right R=0,5,10,15, 40$h^{-1}$ Mpc. The mocks used in this test were in real space. The dashed white line indicates the 1-1 relation. The solid line comes from fitting a 2D-Gaussian to the 2D histogram; it represents the angle between the major axis and the ordinate axis. The angle does not  indicate the bias of the reconstructed displacements compared with the true displacements but provides an illustration of the effect. The best result is obtained for the 10-15 $h^{-1}$ Mpc according to our quantitative results shown in Table \ref{tab:noise_bias_sky}.
%	  The scatter increased because of the inference of the velocity field from the density in redshift space and the noise in the density estimation generated by the geometry of the survey and the decrease in the mean density by 1/10.} }
%	    	\label{fig:hist2dsky_RD}
%\end{figure*}

%{\bf [Tables for QPM bias and error eliminated]}

%\begin{table}
%\begin{center}
%\caption{  Error and bias from equations \ref{eq:postulat}, \ref{eq:alpha} and \ref{eq:sigma}; from 10 reconstructed QPM mocks with different smoothing lengths. The best results  are obtained for the 5$h^{-1}$ Mpc smoothing scale.} 
%\label{tab:noise_bias_norsd}
%\begin{tabular}{@{}lcccccc}
%\hline
%R & $<\mathcal{C}(\tilde{\psi}_R,\psi)>$ & $<\alpha>$ & $\sigma_{\alpha}$ & $<\sigma_N>$ & $\sigma_{\sigma_N}$ & $\frac{<\sigma_N>}{<\alpha>}$   \\
%\hline
%%0 *  & 0.50 &0.42 &-& 6.15&-&8.30\\
%5 & 0.68 & 0.47 &  $<$0.01 & 3.56 & 0.00 & 7.54\\
%10 & 0.67 & 0.37 & $<$0.01 & 2.94 & $<$0.01 & 7.80\\
%15 & 0.63 & 0.31 & $<$0.01 & 2.69 & 0.01 & 8.58\\
%20 & 0.60 & 0.26 & $<$0.01 & 2.51 & 0.01 & 9.39\\
%40 & 0.49 & 0.16 & $<$0.01 & 2.00 & 0.02 & 12.4\\
%\hline
%\\[-1.5ex]
%\end{tabular}
%\end{center}
%\end{table}


\begin{table}
\begin{center}
\caption{ \textbf{PBrun Cubic} Error and bias from equations \ref{eq:postulat}, \ref{eq:alpha} and \ref{eq:sigma}; from 1 reconstructed PBrun Cubic mock with different smoothing lengths. The best results  are obtained for the 5$h^{-1}$ Mpc smoothing scale.}
\label{tab:noise_bias_pbrun}
\begin{tabular}{@{}lcccccc}
\hline
R & $\mathcal{C}(\tilde{\psi}_R,\psi)$ & $\alpha$ & 
$\sigma_N$ & 
$\frac{\sigma_N}{\alpha}$   \\
\hline
%0    & 0.54     &1.61  &    9.77    &   6.07\\
5    & 0.87     &1.01  &    2.23    &   2.21\\
10   &  0.83   &  0.77 &    2.08  &     2.70\\
15    & 0.77&   0.64  &      2.05  &    3.20\\
40    & 0.60 &  0.33 &     1.74  &      5.27\\
\hline
\\[-1.5ex]
\end{tabular}
\end{center}
\end{table}



%\begin{table}
%\begin{center}
%\caption{ \rr{eliminated} \textbf{Sky Mocks} Error and bias from equations \ref{eq:postulat}, \ref{eq:alpha} and \ref{eq:sigma}; from 10 reconstructed QPM sky mocks with different smoothing lengths. The best results are obtained for the 15$h^{-1}$ Mpc smoothing scale.}
%\label{tab:noise_bias_sky}
%\begin{tabular}{@{}lcccccc}
%\hline
%R & $<\mathcal{C}(\tilde{\psi}_R,\psi)>$ & $<\alpha>$ & $\sigma_{\alpha}$ & $<\sigma_N>$ & $\sigma_{\sigma_N}$ & $\frac{<\sigma_N>}{<\alpha>}$   \\
%\hline
%%0 & 0.26 & 2.35 & -&5.4 &-&7.08\\
%5    & 0.41     &0.29  &  0.01   &   3.71    & 0.10    &  13.06\\
%10   &  0.49   &  0.27 &   0.01  &    2.98  &   0.10  &   11.01\\
%15    & 0.50  &   0.24  &  0.01  &    2.58  &   0.11  &    10.76\\
%40    & 0.42 &    0.13   & 0.01 &     1.62  &   0.14  &    12.63\\
%
%\hline
%\\[-1.5ex]
%\end{tabular}
%\end{center}
%\end{table}

\subsubsection{Theoretical Estimation of Bias and Noise}\label{biasrec}
In order to get a sensible estimate of the bias and noise level, we follow an approach in terms of probability distributions. We  write the reconstructed displacement as a biased estimation of the "true" displacement $\psi$ plus a Gaussian noise : 
\begin{equation}
\label{eq:postulat}
\tilde{\psi}_R = \alpha\times\psi + \mathcal{N}(0,\sigma_N),
\end{equation}
where $\alpha$ is the bias term and $\sigma_N$ characterises entirely the noise. Because the noise is uncorrelated to the displacement, then we have:
\begin{equation}
\label{eq:first_rel}
\tilde{\sigma}_R^2 = \alpha^2\sigma_{\psi}^2 + \sigma_N^2,
\end{equation}
where $\tilde{\sigma}_R^2$ is the variance of the "reconstructed" displacements for the smoothing scale $R$ and $\sigma_{\psi}^2$ is the variance of the "true" displacements. We must notice we do not have direct access to  $\alpha$ and $\sigma_N$. The observable quantities are the variance or standard deviation from $\psi$ and $\tilde{\psi}_R$ (i.e. $\sigma_{\psi}$ and $\tilde{\sigma}_R$) and $\tilde{\alpha}$ the angle of the correlation between $\psi$ and $\tilde{\psi}_R$ \footnote{$\tilde{\sigma}_R$ using directly the standard deviation of the reconstructed values. In the case of simulations, we have access to $\sigma_{\psi}$  which is obviously not the case using data.}. 


While the equation (\ref{eq:first_rel}) provides a relation between the observable quantities and the intrinsic bias and noise, we still need to break the degeneracy between the two contributions. We propose to use the scatter plot between $\tilde{\psi}_R$ and $\psi$. Following the calculus of Appendix \ref{ap:biasnoise}, we get the following expressions for the bias of the reconstructed displacements and the associated noise ($\alpha$, $\sigma_N$) for a smoothing scale $R$ given the measurable quantities ($\tilde{\alpha}$, $\sigma_{\psi}$, $\sigma_{\tilde{\psi}_R}$): \begin{equation}
\label{eq:alpha}
\alpha = \frac{\sigma_{\tilde{\psi}_R}^2}{\tilde{\alpha}\sigma_{\psi}^2}.
\end{equation}
\begin{equation}
\sigma_N^2 = \tilde{\sigma}_R^2 - \frac{\tilde{\sigma}_R^4}{\tilde{\alpha}^2\sigma_{\psi}^2}.
\label{eq:sigma}
\end{equation}

The dispersion of the de-biased displacement is then given by $\sigma_N/\alpha$. This quantity enables us to evaluate the quality of the estimator depending only on the smoothing scale $R$, $\sigma_N$ and $\alpha$.



\subsubsection{Measurement of Bias and Noise}\label{biasrecres}
%\rr{I don't think that the bias and noise estimate makes sense in this context. The slope of the distribution i.e. your alpha value depends on the comparative size of the displacement which (as previously) depends on how much the perturbation amplitude is suppressed by the smoothing. The noise is more interesting and I think this should be the quantity that you use to decide the optimal smoothing length or even better would be to smooth the true displacements with the same filter and then compare the distributions. The larger smoothing scale reduces the gradient of the comparative distributions and thus amplifies the stat. sigmaN/alpha. ÊTable 6 and 7 show quite different results for alphaÉalso which mocks in fig. 10. All of this is very confusing. Maybe it would be better to stick to one set of mocks..?I think all of section 6 generally is very confusing. I think you are trying to do too much with too many data sets and nothing is really very clear and some of the tests don't make sense to me. I think this section needs considerable work or removing entirely.}

%\comment{We decided to stick to PBruns, QPM and PBrun are in agreement so this choose does not affect the conclusions of the paper. we decided NOT to eliminated  alpha/noise. We will try to defend our methodology.}

%\bb{SEBASTIEN we need here add a paragraph(s) that answers the referee concerns....}
%The main purpose of this section is to estimate the accuracy of the individual velocityÊobtained using reconstruction and be able to associate an individual error in their estimation (and we need the bias to derive the correct one). Moreover, we provide a quality estimator in perfect agreement with the correlationÊcoefficient results confirming that our analysis is correct but providing twoÊrelevant informations for other studies.


We measure the $\sigma_{\tilde{\psi}_R}$ and $\sigma_{\psi}$ standard deviation from reconstructed and simulation displacements. We measure the correlation coefficient $\mathcal{C}(\tilde{\psi}_R,\psi)$. 
We calculate the biased coefficient $\tilde{\alpha}$:
\begin{equation}
\tilde{\alpha}=\frac{\sigma_{\tilde{\psi}_R}}{\sigma_{\psi} \mathcal{C}(\tilde{\psi}_R,\psi)}
\end{equation} 
We deduce the two quantities, the bias $\alpha$ and the noise, $\sigma_N$, using equations (\ref{eq:alpha}) and (\ref{eq:sigma}). Once we have the values for the bias and the noise, we can determine which smoothing scale is the best. We expect a similar result as the correlation coefficient but knowing the contribution from the intrinsic noise, $\sigma_N$, for the different smoothing scales. We expect a lower noise for the larger smoothing scale as we are deleting more efficiently the nonlinear scales. However, we also expect to have a poorer precision in the displacement reconstruction because we are losing some structures corresponding to the linear theory. So, we expect a lower value for the bias $\alpha$ as we  increase the smoothing scale. The best smoothing scale is therefore the one that balances the two effects and corresponds to the minimum value of the ratio $\sigma_N / \alpha$ as demonstrated in the appendix.

The results are shown in Table %s \ref{tab:noise_bias_norsd} for the QPM cubic mocks in real space and Table % \sout{In Table \ref{tab:noise_bias_sky} we show the results for QPM sky-mocks in redshift space.}
\ref{tab:noise_bias_pbrun} for PBrun cubic mocks in real space. Figure \ref{fig:sumbiasnoise} summarises bias and noise results for the three sets of mocks. Top panel shows the correlation coefficient $<\mathcal{C}(\tilde{\psi}_R,\psi)>$ as a function of the smoothing scale, intermediate panel shows the quality factor $\sigma_N / \alpha$ as a function of the smoothing scale. Finally, bottom panel shows the noise $\sigma$ and the bias $\alpha$ as a function of the smoothing scale.
%We decide to eliminate PBruns just to be treated in another paper. We consider the results of RSD mocks are intriguing and we need more investigation before presenting this results. It is probable that as we are not treating correctly the RSD the results are affected. We decide to make further investigations and eliminate this case from the paper.}
%\begin{itemize}
%
%\item  Real Mocks: the smaller the smoothing scale is, the better the result is. Then, the 5 $h^{-1}$ Mpc scale provides the best ratio $\sigma_N/\alpha$ value as well as the best correlation coefficient value $C=0.68$. However, we can see that the 10$h^{-1}$ Mpc scale have similar results. We can think that the best value could reside between these two scales.
%\item 
%PBrun Mock:  
{\bf  The best results are obtained for the highest correlation coefficient and the lowest quality factor. We find that the quality value is a monotonic function of the smoothing scale. The ratio $\sigma_N/\alpha$ is minimized for $R=5 h^{-1}$ Mpc and also that the maximal correlation coefficient value ($C=0.87$) corresponds to the $R=5 h^{-1}$ Mpc. 
We can see also from the bottom panel of Figure \ref{fig:sumbiasnoise}, that both the bias, $\alpha$, and the noise, $\sigma_N$, are decreasing with the smoothing scale, but at a different ratio. As shown in the appendix B, the ratio is the way to measure the accuracy of the estimator (equation B.10). Figure  \ref{fig:sumbiasnoise} also allows to explain why $R=5 h^{-1}$ Mpc is performing better, while a smaller smoothing results in a improved correlation, the noise level increases more abruptly than the correlation, thus giving a poorer displacement field.
From the top and intermediate panels of Figure  \ref{fig:sumbiasnoise}, we can see that the correlation coefficient and the ratio $\sigma_N/\alpha$ are symmetric and so provide equivalent information. However, while the correlation coefficient provides a single information, with the methodology we proposed, we have access to the bias and the noise of the estimator separately. This point is important when one wants to use the reconstruction methodology to derive the velocity field directly and associate errors to it.}

%\sout{We can see that the correlation coefficient increases significantly compared with the cubic QPM  mocks for all smoothing scales as well as the $\alpha$ values, and the noise levels are also smaller. The results seem to indicate the QPM velocities are noisier compared with the PBrun velocities while the latter are more realistic velocities. }

%\sout{Sky Mocks: unlike the Real Mocks, the quality value is not a monotonic function of the smoothing scale. We find that the ratio $\sigma_N/\alpha$ is minimized for $R=15 h^{-1}$ Mpc. The results are also very similar for the scales $R=10 h^{-1}$ Mpc but the best value seems to be close to $R=15 h^{-1}$ Mpc. We can see that the correlation coefficient decreases significantly for all the interesting scales.}

%\end{itemize}


\begin{figure}
   \centering    
   \includegraphics[width=3.8in]{test_3-1.pdf}%{Plot_tables_paperDR12_coeff.pdf} \includegraphics[width=3.35in]{Plot_tables_paperDR12_SOA.pdf} 	%\bb{Change plot eliminating QPM sky mocks and PBrun} 
   	  \caption{ {\bf Top panel shows the correlation coefficient $<\mathcal{C}(\tilde{\psi}_R,\psi)>$ , central panel the quality factor $\sigma_N / \alpha$, and bottom panel the bias $\alpha$ and the noise $\sigma$, as a function of the smoothing scale. The best results for cubic mocks  PBrun  are for 5 $h^{-1}$ Mpc, while the best result for the Sky mocks are obtained for 10-15 $h^{-1}$ Mpc.}}
	    	\label{fig:sumbiasnoise}
\end{figure}
\subsubsection{Halo Bias Dependence}%\comment{This will be treated in deep in other paper}}

In this section we explore how the conclusions we get for BOSS-like samples in the last section scale for other biases and number densities so the results could be applied to other surveys. We show the effects in terms of the displacement field as the bias effect in the correlation function; anisotropic fits are treated in another appendix. For this test we generate several halo samples from PBrun simulation, applying different halo mass cuts. The samples information  is summarised in the Table \ref{tab:halocut}; we show the number density, shot noise level and halo bias. The halo bias is determined by comparing the power spectrum of halos with the dark matter power spectrum from the simulations.
\begin{table}
\begin{center}
\caption{  PBrun mocks samples generated from different Halo mass cuts. } 
\label{tab:halocut}
\begin{tabular}{@{}lccccc}
\hline
Mcut	 & number density&	 Shot Noise & Halo Bias& $k_{max}$\\	
\hline
1.0e12  & 0.00287320     &348.044 &1.29069 &0.568604\\
3.0e12   &0.00105167     & 950.872&1.55206&0.364857\\
5.0e12  &0.000616345    &  1622.47&1.71838&0.326531 \\
7.0e12  &0.000425321   &   2351.17&1.85922&0.261644\\
9.0e12  &0.000319666   &   3128.27&1.96803&0.234149\\
1.0e13  &0.000281704   &   3549.83&2.02379&0.234149\\
2.0e13  &0.000117975   &   8476.39&2.41207&0.167890\\
3.0e13  &6.69662e-05   &   14932.9&2.71752&0.134476\\
4.0e13  &4.35019e-05  &     22987.5&2.95412& 0.107754\\
5.0e13  &3.05197e-05  &      32765.7&3.14878&0.0964309\\
\hline
\end{tabular}
\end{center}
\end{table}

 We show the scatter plots between true and reconstructed displacements for PBrun Mocks in Figure \ref{fig:hist2dpbruncuts}. Each line of plots represent different halo cuts, i.e represent a sample with a different halo bias. From top to bottom, $M_{halo}=[1e12, 5e12, 9e12, 1e13, 2e13, 4e13, 5e13 ] M \odot$. The different columns show the different smoothing scales, from left to right R=[2,5,10,15,20,40]$h^{-1}$ Mpc. The dashed black line indicates the 1-1 relation. The solid line comes from fitting a 2D-Gaussian to the 2D histogram; it represents the angle between the major axis and the ordinate axis. This angle does not  indicate the bias of the reconstructed displacements compared with the true displacements but provides an illustration of the effect. 

 The results of the bias and noise ( equations \ref{eq:alpha} and \ref{eq:sigma}) are presented in the Table \ref{tab:halocut}. The quality factor and coefficient of correlation indicate for each case what is the best smoothing scale. 
The best results are for the higher correlation coefficient and the lower quality factor.
 The Figure \ref{fig:sumbiasnoisecut} summarises bias and noise results for the samples generated with different halo mass cuts. Right panel shows the correlation coefficient $<\mathcal{C}(\tilde{\psi}_R,\psi)>$ and left panel the quality factor $\sigma_N / \alpha$ as a function of the smoothing scale.
 
 The results for the correlation coefficient and the quality factor show two regimes: 1) For small smoothing scale the result  depends strongly on the bias; 2) For large smoothing scale the results converge in the correlation coefficient and quality factor for all the biases.
These two behaviours could be understood considering number density and shot noise. %The bottom left panel of Figure \ref{fig:sumbiasnoisecut} shows the power spectrum of the different samples and the shot noise level associated to each sample. The bottom right shows the respective bias of the samples for the different halo mass cuts. 
The greater the mass cut is, the greater the bias is and also the greater the shot noise level of the samples. The samples that are more biased, are more affected by the shot noise; for those cases a smoothing scale from 5-10$h^{-1}$ Mpc is preferable, while for low biased tracers a smaller smoothing scale, from 2-5$h^{-1}$ Mpc also gives a good result. 
On the other hand we can see that the result is similar for all the biases for the large smoothing scale, indicating that the smoothing is compensating for the shot noise effect on the reconstructed displacements. 

\begin{table}
\begin{center}
\caption{ PBrun mocks samples for several Halo Mass Cuts.  Error and bias from reconstructed PBrun Cubic mocks  with different smoothing lengths. } 
\label{tab:halocut}
\begin{tabular}{@{}lccccc}
\hline
R & $\mathcal{C}(\tilde{\psi}_R,\psi)$ & $\alpha$ & 
$\sigma_N$ & 
$\frac{\sigma_N}{\alpha}$   \\
\hline
Mass cut = 1.0e12\\
\hline
%2 & 0.87 & 1.05 & 2.31 & 2.19 \\
5 & 0.87 & 0.87 & 1.94 & 2.21 \\
10 & 0.81 & 0.70 & 1.95 & 2.79 \\
15 & 0.76 & 0.58 & 1.93 & 3.31 \\
20 & 0.72 & 0.49 & 1.88 & 3.79 \\
40 & 0.59 & 0.29 & 1.59 & 5.41 \\
\hline
Mass cut = 3.0e12\\
\hline
%2 & 0.85 & 1.13 & 2.73 & 2.41 \\
5 & 0.87 & 0.91 & 2.00 & 2.19 \\
10 & 0.82 & 0.72 & 1.97 & 2.74 \\
15 & 0.77 & 0.59 & 1.95 & 3.27 \\
20 & 0.72 & 0.50 & 1.90 & 3.75 \\
40 & 0.59 & 0.29 & 1.61 & 5.38 \\
\hline
Mass cut = 5.0e12\\
\hline
%2 & 0.83 & 1.20 & 3.12 & 2.59 \\
5 & 0.87 & 0.94 & 2.06 & 2.18 \\
10 & 0.82 & 0.73 & 2.00 & 2.71 \\
15 & 0.77 & 0.60 & 1.96 & 3.23 \\
20 & 0.73 & 0.51 & 1.91 & 3.70 \\
40 & 0.59 & 0.30 & 1.61 & 5.31 \\
\hline
Mass cut = 7.0e12\\
\hline
%2 & 0.81 & 1.25 & 3.46 & 2.76 \\
5 & 0.87 & 0.97 & 2.13 & 2.19 \\
10 & 0.82 & 0.75 & 2.03 & 2.71 \\
15 & 0.77 & 0.61 & 2.00 & 3.23 \\
20 & 0.72 & 0.52 & 1.94 & 3.71 \\
40 & 0.59 & 0.30 & 1.65 & 5.35 \\
\hline
Mass cut = 9.0e12\\
\hline
%2 & 0.80 & 1.30 & 3.80 & 2.90 \\
5 & 0.87 & 0.99 & 2.19 & 2.20 \\
10 & 0.82 & 0.76 & 2.06 & 2.69 \\
15 & 0.77 & 0.62 & 2.02 & 3.22 \\
20 & 0.72 & 0.53 & 1.96 & 3.70 \\
40 & 0.59 & 0.31 & 1.67 & 5.33 \\
\hline
\end{tabular}
\end{center}
\end{table}

\begin{table}
\begin{center}
\caption{ PBrun mocks samples for several Halo Mass Cuts.  Error and bias from reconstructed PBrun Cubic mocks  with different smoothing lengths. } 
\label{tab:halocut2}
\begin{tabular}{@{}lccccc}
\hline
R & $\mathcal{C}(\tilde{\psi}_R,\psi)$ & $\alpha$ & 
$\sigma_N$ & 
$\frac{\sigma_N}{\alpha}$   \\

\hline
Mass cut = 1.0e13\\
\hline
%2 & 0.79 & 1.32 & 3.95 & 2.97 \\
5 & 0.87 & 1.00 & 2.22 & 2.21 \\
10 & 0.82 & 0.76 & 2.06 & 2.69 \\
15 & 0.77 & 0.62 & 2.02 & 3.21 \\
20 & 0.72 & 0.53 & 1.96 & 3.69 \\
40 & 0.59 & 0.31 & 1.67 & 5.32 \\
\hline
Mass cut = 2.0e13\\
\hline
%2 & 0.73 & 1.52 & 5.56 & 3.64 \\
5 & 0.85 & 1.09 & 2.62 & 2.40 \\
10 & 0.81 & 0.80 & 2.20 & 2.74 \\
15 & 0.76 & 0.65 & 2.11 & 3.24 \\
20 & 0.72 & 0.54 & 2.03 & 3.72 \\
40 & 0.59 & 0.31 & 1.70 & 5.35 \\
\hline
Mass cut = 3.0e13\\
\hline
%2 & 0.67 & 1.69 & 7.13 & 4.21 \\
5 & 0.82 & 1.16 & 3.05 & 2.62 \\
10 & 0.81 & 0.83 & 2.34 & 2.80 \\
15 & 0.76 & 0.66 & 2.18 & 3.26 \\
20 & 0.72 & 0.55 & 2.08 & 3.72 \\
40 & 0.59 & 0.32 & 1.73 & 5.32 \\
\hline
Mass cut = 4.0e13\\
\hline
%2 & 0.63 & 1.84 & 8.68 & 4.71 \\
5 & 0.80 & 1.22 & 3.53 & 2.87 \\
10 & 0.80 & 0.86 & 2.50 & 2.91 \\
15 & 0.75 & 0.68 & 2.27 & 3.33 \\
20 & 0.71 & 0.56 & 2.14 & 3.77 \\
40 & 0.58 & 0.32 & 1.75 & 5.35 \\
\hline
Mass cut = 5.0e13\\
\hline
%2 & 0.59 & 1.99 & 10.3 & 5.19 \\
5 & 0.77 & 1.29 & 4.09 & 3.16 \\
10 & 0.78 & 0.88 & 2.71 & 3.07 \\
15 & 0.74 & 0.69 & 2.39 & 3.45 \\
20 & 0.70 & 0.57 & 2.22 & 3.87 \\
40 & 0.58 & 0.32 & 1.77 & 5.41 \\  
\hline
\end{tabular}
\end{center}
\end{table}
\begin{figure*}
   \centering    
\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=2_mcut_1_0e12.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=5_mcut_1_0e12.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=10_mcut_1_0e12.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=15_mcut_1_0e12.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=20_mcut_1_0e12.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=40_mcut_1_0e12.pdf}
\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=2_mcut_5_0e12.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=5_mcut_5_0e12.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=10_mcut_5_0e12.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=15_mcut_5_0e12.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=20_mcut_5_0e12.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=40_mcut_5_0e12.pdf}
%\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=2_mcut_7_0e12.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=5_mcut_7_0e12.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=10_mcut_7_0e12.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=15_mcut_7_0e12.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=20_mcut_7_0e12.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=40_mcut_7_0e12.pdf}
\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=2_mcut_9_0e12.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=5_mcut_9_0e12.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=10_mcut_9_0e12.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=15_mcut_9_0e12.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=20_mcut_9_0e12.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=40_mcut_9_0e12.pdf}
\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=2_mcut_1_0e13.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=5_mcut_1_0e13.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=10_mcut_1_0e13.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=15_mcut_1_0e13.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=20_mcut_1_0e13.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=40_mcut_1_0e13.pdf}
\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=2_mcut_2_0e13.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=5_mcut_2_0e13.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=10_mcut_2_0e13.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=15_mcut_2_0e13.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=20_mcut_2_0e13.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=40_mcut_2_0e13.pdf}
%\includegraphics[width=1.2in]{Paper_Gauss2Dfit_R=2_mcut_3_0e13.pdf}\includegraphics[width=1.2in]{Paper_Gauss2Dfit_R=5_mcut_3_0e13.pdf}\includegraphics[width=1.2in]{Paper_Gauss2Dfit_R=10_mcut_3_0e12.pdf}\includegraphics[width=1.2in]{Paper_Gauss2Dfit_R=15_mcut_3_0e13.pdf}\includegraphics[width=1.2in]{Paper_Gauss2Dfit_R=20_mcut_3_0e12.pdf}\includegraphics[width=1.2in]{Paper_Gauss2Dfit_R=40_mcut_3_0e13.pdf}
\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=2_mcut_4_0e13.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=5_mcut_4_0e13.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=10_mcut_4_0e13.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=15_mcut_4_0e13.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=20_mcut_4_0e13.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=40_mcut_4_0e13.pdf}
\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=2_mcut_5_0e13.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=5_mcut_5_0e13.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=10_mcut_5_0e13.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=15_mcut_5_0e13.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=20_mcut_5_0e13.pdf}\includegraphics[width=1.1in]{Paper_Gauss2Dfit_R=40_mcut_5_0e13.pdf}


	 \caption{We show the scatter plots between true and reconstructed displacements for PBrun Mocks. Each line of plots represents different halo cuts (i.e  represents a sample with a different halo bias). The different columns represent the different smoothing scales, from left to right R=2,5,10,15,20,40$h^{-1}$ Mpc. The mocks used in this test were in real space. The dashed black line indicates the 1-1 relation.
	 The solid line comes from fitting a 2D-Gaussian to the 2D histogram, it represents the angle between the major axis and the ordinate axis. 
	  This angle does not  indicate the bias of the reconstructed displacements compared with the true displacements but provides an illustration of the effect.	  
	  The results of the bias and noise are presented in the Table \ref{tab:noise_bias_norsd}. The  higher correlation coefficient and the lower quality factor indicates the best result for each case.
	  } 

   	\label{fig:hist2dpbruncuts}
\end{figure*}
%

\begin{figure*}
   \centering    
\includegraphics[width=3.3in]{Correl_coeff_RunPB.pdf}\includegraphics[width=3.3in]{SOA_RunPB.pdf}
%\includegraphics[width=3.3in]{Pk_PB00_Halos_total_and_mcuts_WSN.pdf}\includegraphics[width=3.3in]{Bias_PB00_Halos_total_and_mcuts_WSN.pdf}
\caption{ Top left panel shows the correlation coefficient $<\mathcal{C}(\tilde{\psi}_R,\psi)>$ and right top panel the quality factor $\sigma_N / \alpha$ as a function of the smoothing scale. %The bottom left panel shows the power spectrum of the different samples and the shot noise level associated to each sample. The bottom right shows the respective bias of the samples for the different halo mass cuts.
The different samples follow similar trends: the best results are obtained for the higher correlation coefficient and the lower quality factor; using the  5 $h^{-1}$ Mpc smoothing scale gives the best results for the most of the cases. The more biased samples, are more affected by the shot noise  and for those cases, a smoothing scale from 5-10$h^{-1}$ Mpc is preferable, while for low biased tracers a smaller smoothing scale, from 2-5$h^{-1}$ Mpc also gives a good result. On the other hand we can see that the result is similar for all the biases for the large smoothing scale, indicating that the smoothing is compensating for the shot noise effect on the reconstructed displacements. }
	\label{fig:sumbiasnoisecut}
\end{figure*}

\section{Conclusion}\label{sec:con}
%\rr{I would disagree with your main conclusion that the best smoothing length is 5Mpc/h. I would remove the R=0 case.}

We summarize the results presented in this paper.

\begin{itemize}
\item We test reconstruction algorithm using five different smoothing scales $5$, $10,15$, $40 h^{-1}Mpc$ with QPM BOSS-like mock {\bf catalogues} and we study the effect in BAO anisotropic analysis.
 We find that the different smoothing scales affect the multipoles. We observe variations in the amplitude of the monopole a low scales and in the sharpening of the BAO feature. The effects on the quadrupole are larger than in the monopole. The smoothing scale of 15 $h^{-1}$ Mpc produces a quadrupole not completely consistent with zero. Taking a smaller smoothing scale reduces the negative correlation observed in the quadrupole to be in agreement with zero  within the fitting range. A large smoothing scale increases the negative correlation in the quadrupole at scales between $50-100 h^{-1}$Mpc.
 \item We show that the smoothing scale affects the anisotropic clustering results. {\bf The results indicate that the best choice for the smoothing length, in terms of anisotropic clustering, is given by the smaller smoothing scale of $5 h^{-1}Mpc$.  This smoothing scale shows the smaller bias and error  on $\alpha$ an $\epsilon$ error bars simultaneously}. The variations in the mean value for best fits parameters using $15 h^{-1}$ Mpc compared with $5h^{-1}$ Mpc are
$\sim$0.5\% for $\alpha$ and 0.3 for $\epsilon$, producing $\Delta D_A , \Delta H\sim 0.5$\%. 
 The smoothing scale affects the precision at which we can measure the BAO parameters. Taking $15 h^{-1}$Mpc as a reference, the median error using 5 Mpc/h is reduced by 10\% for $\alpha$ and 45\% for $\epsilon$. The  effect on the uncertainties of DA(z) and H(z) are 40\% and 30\% respectively.
%\item We show that the smoothing scale affects the anisotropic clustering results.  The results indicate that the best choice for the smoothing length, in terms of anisotropic clustering, is given by the smaller smoothing scale of $5 h^{-1}Mpc$, given the smaller bias and error bars for this smoothing scale. The variations in the mean value for best fits parameters using $15 h^{-1}$ Mpc compared with $5h^{-1}$ Mpc are $\sim$0.5\% for $\alpha$ and 0.3 for $\epsilon$, producing $\Delta D_A , \Delta H\sim 0.5$\%. The smoothing scale affects the precision at which we can measure the BAO parameters. Taking $15 h^{-1}$Mpc as a reference, the median error using 5 Mpc/h is reduced by 10\% for $\alpha$ and 45\% for $\epsilon$. The  effect on the uncertainties of DA(z) and H(z) are 40\% and 30\% respectively.
\item We explore the effect of the smoothing scale in the reconstructed displacement field to investigate our hypothesis, i.e. if the improvement observed in the post-reconstruction anisotropic clustering was coming from a better estimation of the displacement field when we reduce the smoothing scale. {\bf We studied first, the coefficient of cross-correlation between true and reconstructed displacements fields for cubic mocks in real space. }%For the displacement distribution, we find that, we get a better match to the simulation distribution for the $5 h^{-1}$ Mpc smoothing scale.
  %For the coefficient of correlation, 
  We found the correlation  improves (i.e. gets closer to 1)  for the 5 $h^{-1}$ Mpc smoothing scale for larger values of k; this verifies the fact that the displacements recovered in reconstruction are better correlated with the true displacements for this smoothing scale. We also estimate the error and bias of reconstructed displacements, comparing the  true displacements from simulations to the reconstructed displacements. 
{\bf   We find that the quality value, $\sigma_N/\alpha$ is minimized for $R=5 h^{-1}$ Mpc and also that the maximal correlation coefficient value ($C=0.9$) corresponds to the $R=5 h^{-1}$ Mpc. }
 % We found the best agreement using 5 $h^{-1}$ Mpc  for cubic mocks in real space for PBrun. 
  %\sout{both sets of mocks (QP} PBrun.  We measure a correlation coefficient between true and reconstruction displacements of \sout{0.7 for cubic QPM in real space ,} 0.9 for PBrun mocks in real space.
  %{\bf    We measure a correlation coefficient between true and reconstruction displacements of %\sout{0.7 for cubic QPM in real space ,}
%   0.9 for PBrun mocks in real space.}
%\item   \sout{ We also study also our hypothesis in the case of sky mocks. Unfortunately, we found that when we included the redshift distortions and bias, we get a different optimal smoothing compared to the cubic mocks. We found that a smoothing scale between 10-15 $h^{-1}$ is better for sky mocks. This result indicates that the improvement of the anisotropic fits with a smaller smoothing scale is not related to a better agreement in the displacement field. We measure a correlation coefficient between true and reconstruction displacements of  0.5 for QPM sky mocks in redshift space. This characterisation of the error for displacement field can be useful if we are interested in using the reconstructed velocity field for cosmology projects other than BAO analysis.}
 \item  We explore how the conclusions we get for BOSS-like samples scale for other bias and number densities so the results could be applied to other surveys. We show the effects in terms of the displacement field (and in the appendix the bias effect in the correlation function). For this test we generate several halo samples from PBrun simulation, applying different halo mass cuts.The results for the correlation coefficient and the quality factor show two regimes: 1) For small smoothing scale the result  depends strongly on the bias;  the samples that are more biased, are more affected by the shot noise; for those cases a smoothing scale from 5-10$h^{-1}$ Mpc is preferable, while for low biased tracers a smaller smoothing scale, from 2-5$h^{-1}$ Mpc also gives a good result. 2) For large smoothing scale the results converge in the correlation coefficient and quality factor for all the biases, indicating that the smoothing is compensating for the shot noise effect on the reconstructed displacements, and the dependence on bias is weaker.
 
 \end{itemize}
 Further work should be done to provide a theoretical framework to the empirical results shown in this article. 
 The optimal smoothing scale could vary for different tracers (different kinds of galaxies) or could maybe also depend on the redshift and environmental properties. A future work will  be focus on exploring these different dependencies to look for ways to improve the reconstruction technique for future surveys such as eBOSS, DESI, EUCLID. 
\section{Acknowledgements}
Many thanks to Nikhil Padmanabhan and Angela Burden for useful discussions and correspondence.

Funding for SDSS-III has been provided by the Alfred P. Sloan Foundation, the Participating Institutions, the National Science Foundation, and the U.S. Department of Energy Office of Science. The SDSS-III web site is http://www.sdss3.org/.
SDSS-III is managed by the Astrophysical Research Consortium for the Participating Institutions of the SDSS-III Collaboration including the University of Arizona, the Brazilian Participation Group, Brookhaven National Laboratory, Carnegie Mellon University, University of Florida, the French Participation Group, the German Participation Group, Harvard University, the Instituto de Astrofisica de Canarias, the Michigan State/Notre Dame/JINA Participation Group, Johns Hopkins University, Lawrence Berkeley National Laboratory, Max Planck Institute for Astrophysics, Max Planck Institute for Extraterrestrial Physics, New Mexico State University, New York University, Ohio State University, Pennsylvania State University, University of Portsmouth, Princeton University, the Spanish Participation Group, University of Tokyo, University of Utah, Vanderbilt University, University of Virginia, University of Washington, and Yale University.

This research used resources of the National Energy Research Scientific Computing Center, a DOE Office of Science User Facility supported by the Office of Science of the U.S. Department of Energy under Contract No. DE-AC02-05CH11231.

\input{ReconstructionSmoothBib_smoo}
\appendix
\section{Comparison of Different Reconstruction Implementations.}\label{ap:imp}
In this section we show that the results obtained in this work are independent of the particular implementation of reconstruction algorithm. We compare our implementation of the reconstruction algorithm (hereafter ``RV") to the method implemented by \cite{Pad12}, hereafter denoted ``RP". The differences between the two methods could be summarised as follows:
\begin{itemize}
\item Solution of Displacement Field. RV implementation solves the 
Poisson equation in Fourier Space assuming real space density field, RP in configuration space using finite differences technique.
\item Redshift Space Corrections. RV neglects the redshift space corrections, while RP takes them into account. This choice is tested to give the accuracy required for BAO anisotropic analysis at sub percent precision in Vargas-Magana (in prep). The corrections are not important because the effect on the quadrupole is a change of the amplitude, and the peak position and contrast are not affected.
\item Survey Mask and Density Estimate. Both methods follow different methods for dealing with the effect of geometry. 
\end{itemize}
We used the same 100 mocks described before and we run reconstruction with RP and RV implementation using the same parameters. We use for this test a bias=2.1 instead of bias=1.87 because the reconstructed {\bf catalogues} were available only for this value of the bias for the RP implementations. We compare results in terms of the multipoles and anisotropic fits. We show in Figure \ref{fig:mean_smooth_bias21} the mean multipoles for the different implementations using three different smoothing lengths, 5, 10, and 15 $h^{-1}$ Mpc. We observe that the monopole behaviour is pretty similar between different implementations in the range of the fitting; the differences observed are only important at scales smaller than 20 $h^{-1}$ Mpc. In the case of the quadrupole,  the amplitude of the quadrupole between different implementations is significantly different. The quadrupole for RP implementation seems to over-correct the anisotropy, while it seems to be under-correcting in our implementation; however, both quadrupoles are very similar in shape. Differences in the quadrupole are generated by two effects: redshift distortions correction and effects of the angular and radial selection functions that are implemented in slightly different ways. Further exploration and quantification of these two contributions which generates differences in the quadrupole amplitude are treated in Vargas-Maga\~na et al (in prep).
\begin{figure}
   \centering    
              \includegraphics[width=1.7in]{Mean_QPM_PostRec_smoothingX0zoomv2_paper.pdf}\includegraphics[width=1.7in]{Mean_QPM_PostRec_smoothingX2v2_paper.pdf} 
  \caption{Multipoles for different smoothing scales: $5,10$ and  15 $h^{-1}$ Mpc for different implementations: in cyan 5 $h^{-1}$ Mpc, in blue 10 $h^{-1}$ Mpc in black 15 $h^{-1}$ Mpc for our implementation. In yellow 5 $h^{-1}$ Mpc, in green 10 $h^{-1}$ Mpc and red 15 $h^{-1}$ Mpc for Padmanabhan et al implementation. In the monopole we observe that, in the fitting region both implementations perform similarly; however, there are some differences at very small scales ($<20 $$h^{-1}$ Mpc). For the quadrupole we observe  important differences in the amplitude. The quadrupole for Padmanabhan et al seems to be kind of over-correcting, while in our implementation seems to be under-correcting; however, both quadrupoles are very similar in shape. Differences in the quadrupole are generated by two effects: redshift distortions correction and effects of the angular and radial selection functions that are implemented in slightly different ways. Further exploration and quantification of these two contributions, which generates differences in the quadrupole amplitude, are treated in Vargas-Maga\~na et al (in prep).}
   \label{fig:mean_smooth_bias21}
\end{figure}

Tables \ref{tab:fittingcomp} and \ref{tab:fittingerrors} summarise the best fitting results. The first table refers to the best fits of $\alpha$ and $\epsilon$ as well as their variance. In the second table we show the mean values of the errors and the RMS of the error distributions.  Additionally, Figures \ref{fig:smoothing_fits} and \ref{fig:smoothing_fitserrors} show the comparison between both implementation's best fits parameters and errors (mean and RMS). The differences between the mean of two different implementations is  ~0.1\% for $\alpha$ and $\epsilon$, indicating the results are completely consistent between both implementations. Also the RMS of the best fits are similar at 0.1\% in both quantities. 

Concerning the errors, the dispersion of the distributions are about the same; however, it seems  to be a systematic larger error in RP implementation compared to RV in $\alpha$ and $\epsilon$. Although the trends are observed in both implementations, the error in $\epsilon$ is monotonically decreasing as we apply a smaller smoothing scale.  In the case of $\alpha$ the errors we get with 5 and 10 $h^{-1}$ Mpc smoothing scale are very similar but smaller than using the 15 $h^{-1}$ Mpc that is regularly applied in BAO analysis.

\begin{table}
\begin{center}
\caption{Best fits. Mean and RMS from 100 reconstructed QPM NGC mocks for different Reconstruction Implementations. } 
\label{tab:fittingcomp}
\begin{tabular}{@{}lccccccccccccc}
\hline
$\Sigma$&
$\widetilde{\alpha}$&RMS&
$\widetilde{\epsilon}$&RMS\\
\hline
This work \\
\hline
5&
$0.9961$&$0.0091$&
$0.0036$&$0.0098$\\
\\[-1.5ex]

10&
$0.9980$&$0.0096$&
$0.0023$&$0.0107$\\
\\[-1.5ex]

15&
$1.0040$&$0.0095$&
$0.0050$&$0.0135$\\


\hline
Padmanabhan et al \\
\hline
5&
$0.9970$&$0.0100$&
$-0.0002$&$0.0088$\\
\\[-1.5ex]

10&
$0.9991$&$0.0116$&
$0.0022$&$0.0112$\\
\\[-1.5ex]

15&
$1.0053$&$0.0107$&
$0.0036$&$0.0141$\\


\hline

 \\[-1.5ex]
\end{tabular}
\end{center}
\end{table}


\begin{table}
\begin{center}
\caption{  Uncertainties on the best fits. Mean, RMS from 100 reconstructed QPM NGC mocks different Reconstruction Implementations. } 
\label{tab:fittingerrors}
\begin{tabular}{@{}lccccccccccccc}
\hline
$\Sigma$&
$\widetilde{\sigma_\alpha}$&RMS&
$\widetilde{\sigma_\epsilon}$&RMS\\
\hline
This work. \\
\hline
5&
$0.0158$&$0.0054$&
$0.0194$&$0.0082$& \\
\\[-1.5ex]
10&
$0.0151$&$0.0044$&
$0.0199$&$0.0071$\\
\\[-1.5ex]
15&
$0.0163$&$0.0051$&
$0.0271$&$0.0084$\\


\hline
Padmanabhan et al \\
\hline
5&
$0.0171$&$0.0063$&
$0.0186$&$0.0090$\\
\\[-1.5ex]
10&
$0.0185$&$0.0049$&
$0.0212$&$0.0070$\\
\\[-1.5ex]
15&
$0.0186$&$0.0051$&
$0.0277$&$0.0076$&\\

\hline
\end{tabular}
\end{center}
\end{table}

\begin{figure}
   \centering   
\includegraphics[width=1.6in]{Smoothing_Fitting_results_alpha_comp2.pdf}
\includegraphics[width=1.6in]{Smoothing_Fitting_results_epsilon_comp2.pdf} 
\caption{Smoothing Fitting Results. Right panel, mean $\alpha$ and RMS of $\alpha$ distribution [right]. Left panel, mean $\epsilon$ and RMS for both implementations. We use a value of the bias=2.1 different than the value used in the article, i.e bias=1.87}   
\label{fig:smoothing_fits}
\end{figure}



\begin{figure}
   \centering   

\includegraphics[width=1.6in]{Smoothing_Fitting_results_sigmaalpha_comp.pdf}\includegraphics[width=1.6in]{Smoothing_Fitting_results_sigmaepsilon_comp.pdf}

\caption{Smoothing Fitting Results.Right, mean $\sigma_\alpha$ and RMS of $\sigma_\alpha$ distribution [right]. Left mean $\sigma_\epsilon$ and RMS for both implementations. We use a value of the bias=2.1 different than the value used in the article, i.e bias=1.87}.

   \label{fig:smoothing_fitserrors}
\end{figure}

Finally in Figure \ref{fig:bias_fits_dep} we put together the results from Section \ref{sec:anisofits} and the results from this section for the anisotropic fits using the same methodology but varying the bias from b=1.87 to b=2.1. The results show that the bias is not affecting the best fits, i.e, the conclusions we get for the smoothing scales in terms of anisotropic results are valid even considering other bias values. 
It is interesting to mention that even when comparing Figures \ref{fig:meanSmooth} and \ref{fig:mean_smooth_bias21}, we observe that, the bias affects the quadrupole amplitude post-reconstruction, this does not affect the best fitting values. 
The uncertainties are shown in Figure \ref{fig:bias_fits_dep2} for both bias values. We observe that the distributions of the uncertainties are quite similar for 10-15 $h^{-1}$ Mpc smoothing scale for both $\alpha$ and $\epsilon$ distributions; however, the lower smoothing scale shows a large dispersion using the bias=1.87 compared to the bias=2.1. This result seems to show that the bias can play a role  in the uncertainties determination when using small smoothing scales. 

\begin{figure}
   \centering   
\includegraphics[width=2.5in]{BestFitsSmoothingResults_alphaepsilon_bias187_21.pdf}
%\includegraphics[width=2.5in]{BestFitsSmoothingResults_alphaepsilon_bias187_21_errors.pdf}
\caption{Smoothing Fitting Results. Top panel, mean $\alpha$ and RMS of $\alpha$ distribution [right]. Bottom panel, mean $\epsilon$ and RMS for two values of the bias=1.87 and bias=2.1. Best fits and dispersion are similar for both values of the bias for all the smoothing scales.} 
   \label{fig:bias_fits_dep}
\end{figure}


\begin{figure}
   \centering   
%\includegraphics[width=2.5in]{BestFitsSmoothingResults_alphaepsilon_bias187_21.pdf}
\includegraphics[width=2.5in]{BestFitsSmoothingResults_alphaepsilon_bias187_21_errors.pdf}
\caption{Smoothing Fitting Results. Top panel, mean $\sigma_\alpha$ and RMS of $\sigma_\alpha$ distribution [right]. Bottom panel, mean $\sigma_\epsilon$ and RMS $\sigma_\epsilon$ distribution  for for two values of the bias=1.87 and bias=2.1. There is a large difference in the dispersion of the $\alpha$ and $\epsilon$ distributions for the lower smoothing scale; however, for 10-15 $h^{-1}$ Mpc, the results are consistent between both bias values.} 
   \label{fig:bias_fits_dep2}
\end{figure}

\section{Bias and Noise Determination}\label{ap:biasnoise}
While the equation (\ref{eq:postulat}) provides us a relation between the variances of reconstructed and true displacement, we need to break the degeneracy between the bias $\alpha$ and the noise effect. We propose to use the correlation plot between $\tilde{\Psi}_R$ and $\Psi$.
We will express the theoretical probability distribution $\mathcal{P}(\tilde{\psi}_R,\psi)$ knowing\footnote{$\sigma_{\psi}$ is a measured quantity and so is known to} the bias $\alpha$, the noise standard deviation $\sigma_N$.


\begin{equation}
\mathcal{P}(\tilde{\psi}_R,\psi) = \mathcal{P}(\psi)\times\mathcal{P}(\tilde{\psi}_R|\psi).
\end{equation}
Assuming a Gaussian distribution, we can express the probability distribution of the``true" displacements  by: 
\begin{equation}
\mathcal{P}(\psi) = \frac{1}{\sqrt{2\pi}\sigma_{\psi}}\exp\left\{-\frac{\psi^2}{2\sigma_{\psi}^2}\right\}.
\end{equation}

Using the relation expressed in equation (\ref{eq:postulat}) we can get the expression for the conditional probability distribution $\mathcal{P}(\tilde{\psi}_R,\psi)$:

\begin{equation}
\mathcal{P}(\tilde{\psi}_R,\psi) = \frac{1}{2\pi\sigma_{\psi}\sigma_{N}}\exp\left\{-\frac{1}{2}\left[\frac{\psi^2}{\sigma_{\psi}^2}+\frac{(\tilde{\psi}_R-\alpha\psi)^2}{\sigma_{N}^2}\right]\right\}.
\end{equation}

The relation we expect to measure between $\tilde{\psi}_R$ and $\psi$ is where $\mathcal{P}(\tilde{\psi}_R,\psi)$ is maximum depending on $\tilde{\psi}_R$ value, i .e. we are interested in the value $\psi_{max}$ which maximises the exponential term for a given $\tilde{\psi}_R$. Then we use the partial derivation:
\begin{equation}
\left.\frac{\partial }{\partial_{\psi}} \left(\frac{\psi^2}{\sigma_{\psi}^2}+\frac{(\tilde{\psi}_R-\alpha\psi)^2}{\sigma_{N}^2}\right)\right|_{\tilde{\psi}_R} = 0.
\end{equation}


Developing this calculus, we obtain the following expression for $\psi_{max}$:
\begin{equation}
\psi_{max} = \frac{\alpha\tilde{\psi}_R}{\frac{\sigma_N^2}{\sigma_{\psi}^2} + \alpha^2 },
\label{eq:rel_psi_max}
\end{equation}
and so $\tilde{\alpha}$ is given by:
\begin{equation}
\tilde{\psi}_R = \tilde{\alpha} \psi_{max} \Rightarrow\tilde{\alpha} = \frac{ \frac{\sigma_N^2}{\sigma_{\psi}^2} + \alpha^2  }{\alpha}.
\label{eq:second_rel}
\end{equation}

We find the relation between $\tilde{\psi}_R$ and $\psi_{max}$ which can be think thought of as representing the apparently most correlated value.  

The 2D correlation provides us an estimation of the bias $\tilde{\alpha}$ which is different than $\alpha$ except for a null noise term $\sigma_N = 0$. 

We have two independent equations (Eq.\ref{eq:first_rel} and Eq.\ref{eq:second_rel} ) which connect ($\alpha$, $\sigma_N$) to the measurable quantities ($\tilde{\alpha}$, $\sigma_{\psi}$, $\sigma_{\tilde{\psi}_R}$).

Combining  Eq.\ref{eq:second_rel}  and Eq.\ref{eq:first_rel}:
\begin{equation}
\label{eqa:alpha}
\alpha = \frac{\sigma_{\tilde{\psi}_R}^2}{\tilde{\alpha}\sigma_{\psi}^2}, 
\end{equation}
and

\begin{equation}
\sigma_N^2 = \tilde{\sigma}_R^2 - \frac{\tilde{\sigma}_R^4}{\tilde{\alpha}^2\sigma_{\psi}^2}.
\label{eqa:sigma}
\end{equation}
We present the comparison between this calculus and measurements in Figure \ref{fig:plot2D}. The plot shows the $\mathcal{P}(\tilde{\psi}_R,\psi)$ for $\alpha=0.5$, $\sigma_N=8$ and $\sigma_{\psi}=10$. The dashed white line represents the relation between $\tilde{\psi}_R$ and $\psi$ without noise term (so $\alpha$), the solid white line represents the theoretical relation obtained using Eq.\ref{eq:second_rel}  (so $\tilde{\alpha}$); the solid red line represent the major axis orientation using a 2D-Gaussian fit. The yellow points correspond respectively to the measured $\psi_{max}(\tilde{\psi}_R)$ on the left and the mean value $\left<\psi(\tilde{\psi}_R)\right>$ on the right panel. From these tests we conclude that the bias and noise estimation described below describes the bias and noise levels observed in our Monte-Carlo realisations.

We can write the de-biased estimator $\overset{D}{\psi_R}$ inverting Eq (\ref{eq:postulat}): 
\begin{equation}
\overset{D}{\psi_R} = \psi+\frac{\mathcal{N}(0,\sigma_N)}{\alpha}.
\end{equation}
Also we can write the dispersion on the de-biased reconstruction as:
\begin{equation}
\overset{D}{\psi_R} - \psi =  \frac{\mathcal{N}(0,\sigma_N)}{\alpha}
\end{equation}


\begin{figure} 
\centering
 \includegraphics[width=1.6in]{test_theory_bias_ellipse_max_alpha=05.pdf}\includegraphics[width=1.6in]{test_theory_bias_ellipse_mean_alpha=05.pdf}
        
  \caption{$\mathcal{P}(\tilde{\psi}_R,\psi)$ for $\alpha=0.5$, $\sigma_N=8$ and $\sigma_{\psi}=10$. The dashed white line represents the relation between $\tilde{\psi}_R$ and $\psi$ without noise term (so $\alpha$), the solid white line represents the theoretical relation obtained using Eq.\ref{eq:second_rel}  (so $\tilde{\alpha}$); the solid red line represents the major axis orientation using a 2D-Gaussian fit. The yellow losanges correspond respectively to the measured $\psi_{max}(\tilde{\psi}_R)$ on the left and the mean value $\left<\psi(\tilde{\psi}_R)\right>$ on the right panel.}
   \label{fig:plot2D}
\end{figure}

\begin{figure} 
\centering
 \includegraphics[width=1.6in]{test_theory_bias_ellipse_max_alpha=08.pdf}\includegraphics[width=1.6in]{test_theory_bias_ellipse_mean_alpha=08.pdf}
        
  \caption{$\mathcal{P}(\tilde{\psi}_R,\psi)$ for $alpha=0.8$, $\sigma_N=8$ and $\sigma_{\psi}=10$. The dashed white line represents the relation between $\tilde{\psi}_R$ and $\psi$ without noise term (so $\alpha$), the solid white line represents the theoretical relation obtained using Eq.\ref{eq:second_rel}  (so $\tilde{\alpha}$); the solid red line represents the major axis orientation using a 2D-Gaussian fit. The yellow losanges correspond respectively to the measured $\psi_{max}(\tilde{\psi}_R)$ on the left and the mean value $\left<\psi(\tilde{\psi}_R)\right>$ on the right panel.}
   \label{fig:plot2D_08}
\end{figure}





